ReFine: Re-randomization before Fine-tuning for Cross-domain Few-shot Learning

Cross-domain few-shot learning (CD-FSL), where there are few target samples under extreme differences between source and target domains, has recently attracted huge attention. Recent studies on CD-FSL generally focus on transfer learning based approaches, where a neural network is pre-trained on popular labeled source domain datasets and then transferred to target domain data. Although the labeled datasets may provide suitable initial parameters for the target data, the domain difference between the source and target might hinder fine-tuning on the target domain. This paper proposes a simple yet powerful method that re-randomizes the parameters fitted on the source domain before adapting to the target data. The re-randomization resets source-specific parameters of the source pre-trained model and thus facilitates fine-tuning on the target domain, improving few-shot performance.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> tables/BN_ablation.tex <==

% \begin{table*}[t]
% \caption{BN ablation study.}
% \addtolength{\tabcolsep}{-4pt}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{c|cc|cc|cc|cc|cc}
%     \hline
%     Track BN Stats & \multicolumn{2}{c|}{miniImageNet} & \multicolumn{2}{c|}{CropDisease} & \multicolumn{2}{c|}{EuroSAT} & \multicolumn{2}{c|}{ISIC} & \multicolumn{2}{c}{ChestX} \\
%     (Pre-train)-(Fine-tune) & 5way-1shot & 5way-5shot & 5way-1shot & 5way-5shot & 5way-1shot & 5way-5shot & 5way-1shot & 5way-5shot & 5way-1shot & 5way-5shot \\
%     \hline 
%     True-True (Baseline) & 44.83 {\stdfont $\pm$ .75} & 73.88 {\stdfont $\pm$ .64} & 57.57 {\stdfont $\pm$ .90} & 88.04 {\stdfont $\pm$ .56} & 51.54 {\stdfont $\pm$ .85} & 79.33 {\stdfont $\pm$ .62} & 32.31 {\stdfont $\pm$ .55} & 49.67 {\stdfont $\pm$ .60} & 21.82 {\stdfont $\pm$ .35} & 26.10 {\stdfont $\pm$ .44} \\
%     True-StatsInit-True  & 44.72 {\stdfont $\pm$ .76} & 73.78 {\stdfont $\pm$ .65} & 57.50 {\stdfont $\pm$ .92} & 88.09 {\stdfont $\pm$ .56} & 51.93 {\stdfont $\pm$ .84} & 79.43 {\stdfont $\pm$ .59} & 31.85 {\stdfont $\pm$ .57} & 50.02 {\stdfont $\pm$ .61} & 22.09 {\stdfont $\pm$ .37} & 25.74 {\stdfont $\pm$ .40} \\
%     % True-StatsInit-False & xx.xx {\stdfont $\pm$ .xx} & xx.xx {\stdfont $\pm$ .xx} & xx.xx {\stdfont $\pm$ .xx} & xx.xx {\stdfont $\pm$ .xx} & xx.xx {\stdfont $\pm$ .xx} & xx.xx {\stdfont $\pm$ .xx} & xx.xx {\stdfont $\pm$ .xx} & xx.xx {\stdfont $\pm$ .xx} & xx.xx {\stdfont $\pm$ .xx} & xx.xx {\stdfont $\pm$ .xx} \\
%     True-False           & 48.44 {\stdfont $\pm$ .77} & 73.98 {\stdfont $\pm$ .66} & 59.74 {\stdfont $\pm$ .90} & 89.03 {\stdfont $\pm$ .56} & 57.30 {\stdfont $\pm$ .84} & 82.12 {\stdfont $\pm$ .60} & 33.75 {\stdfont $\pm$ .61} & 50.88 {\stdfont $\pm$ .60} & 21.83 {\stdfont $\pm$ .37} & 26.05 {\stdfont $\pm$ .41} \\
%     False-True           & 45.41 {\stdfont $\pm$ .74} & 74.35 {\stdfont $\pm$ .65} & 60.42 {\stdfont $\pm$ .93} & 88.77 {\stdfont $\pm$ .56} & 52.86 {\stdfont $\pm$ .84} & 79.45 {\stdfont $\pm$ .60} & 32.32 {\stdfont $\pm$ .58} & 49.20 {\stdfont $\pm$ .59} & 21.86 {\stdfont $\pm$ .37} & 25.35 {\stdfont $\pm$ .41} \\
%     False-False (Ours)   & 48.83 {\stdfont $\pm$ .77} & 75.82 {\stdfont $\pm$ .62} & 62.64 {\stdfont $\pm$ .93} & 90.20 {\stdfont $\pm$ .53} & 58.61 {\stdfont $\pm$ .85} & 82.52 {\stdfont $\pm$ .57} & 33.26 {\stdfont $\pm$ .59} & 50.78 {\stdfont $\pm$ .61} & 22.05 {\stdfont $\pm$ .36} & 25.73 {\stdfont $\pm$ .42} \\
%     \hline
%     \end{tabular} 
% }\label{tab:BN_abla}
% \end{table*}




% \begin{table*}[t]
% \caption{Ablation study on whether statistics are accumulated (AC) or not (NAC) in BN layers. PT and FT stand for pre-training and fine-tuning, respectively.}
% \addtolength{\tabcolsep}{-4pt}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l|cc|cc|cc|cc|cc|cc}
%     \hline
%     \multirow{2}{*}{Method} &
%     \multicolumn{2}{c|}{Accum. Stats.} & \multicolumn{2}{c|}{miniImageNet} & \multicolumn{2}{c|}{CropDisease} & \multicolumn{2}{c|}{EuroSAT} & \multicolumn{2}{c|}{ISIC} & \multicolumn{2}{c}{ChestX} \\
%     & Source & Target & 5way-1shot & 5way-5shot & 5way-1shot & 5way-5shot & 5way-1shot & 5way-5shot & 5way-1shot & 5way-5shot & 5way-1shot & 5way-5shot \\
%     \hline 
%     AC-AC&\cmark & \cmark & 44.83 {\stdfont $\pm$ .75} & 73.88 {\stdfont $\pm$ .64} & 57.57 {\stdfont $\pm$ .90} & 88.04 {\stdfont $\pm$ .56} & 51.54 {\stdfont $\pm$ .85} & 79.33 {\stdfont $\pm$ .62} & 32.31 {\stdfont $\pm$ .55} & 49.67 {\stdfont $\pm$ .60} & 21.82 {\stdfont $\pm$ .35} & 26.10 {\stdfont $\pm$ .44} \\
%     NAC-AC& & \cmark & 45.41 {\stdfont $\pm$ .74} & 74.35 {\stdfont $\pm$ .65} & 60.42 {\stdfont $\pm$ .93} & 88.77 {\stdfont $\pm$ .56} & 52.86 {\stdfont $\pm$ .84} & 79.45 {\stdfont $\pm$ .60} & 32.32 {\stdfont $\pm$ .58} & 49.20 {\stdfont $\pm$ .59} & 21.86 {\stdfont $\pm$ .37} & 25.35 {\stdfont $\pm$ .41} \\
%     NAC-NAC&& & 48.83 {\stdfont $\pm$ .77} & 75.82 {\stdfont $\pm$ .62} & 62.64 {\stdfont $\pm$ .93} & 90.20 {\stdfont $\pm$ .53} & 58.61 {\stdfont $\pm$ .85} & 82.52 {\stdfont $\pm$ .57} & 33.26 {\stdfont $\pm$ .59} & 50.78 {\stdfont $\pm$ .61} & 22.05 {\stdfont $\pm$ .36} & 25.73 {\stdfont $\pm$ .42} \\
%     \hline
%     \end{tabular} 
% }\label{tab:BN_abla}
% \end{table*}


\begin{table}[h]
\caption{Ablation study on whether statistics are accumulated (AC) or not (NAC) in BN layers. PT and FT stand for pre-training and fine-tuning, respectively.}
\addtolength{\tabcolsep}{-4pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|cc|cc|cc}
    \hline
    \multirow{2}{*}{Method} & \multicolumn{2}{c|}{Accum. Stats.} & 1shot & 5shot & 1shot & 5shot \\ \cline{2-7}
    & Source & Target & \multicolumn{2}{c|}{CropDisease} & \multicolumn{2}{c}{EuroSAT} \\
    \hline 
    AC-AC   &\cmark & \cmark & 57.57 {\stdfont $\pm$ .90} & 88.04 {\stdfont $\pm$ .56} & 51.54 {\stdfont $\pm$ .85} & 79.33 {\stdfont $\pm$ .62} \\
    NAC-AC  &       & \cmark & 60.42 {\stdfont $\pm$ .93} & 88.77 {\stdfont $\pm$ .56} & 52.86 {\stdfont $\pm$ .84} & 79.45 {\stdfont $\pm$ .60} \\
    NAC-NAC &       &        & 62.64 {\stdfont $\pm$ .93} & 90.20 {\stdfont $\pm$ .53} & 58.61 {\stdfont $\pm$ .85} & 82.52 {\stdfont $\pm$ .57} \\
    \hline
     &  &  & \multicolumn{2}{c|}{ISIC} & \multicolumn{2}{c}{ChestX} \\
    \hline 
    AC-AC   &\cmark & \cmark & 32.31 {\stdfont $\pm$ .55} & 49.67 {\stdfont $\pm$ .60} & 21.82 {\stdfont $\pm$ .35} & 26.10 {\stdfont $\pm$ .44} \\
    NAC-AC  &       & \cmark & 32.32 {\stdfont $\pm$ .58} & 49.20 {\stdfont $\pm$ .59} & 21.86 {\stdfont $\pm$ .37} & 25.35 {\stdfont $\pm$ .41} \\
    NAC-NAC &       &        & 33.26 {\stdfont $\pm$ .59} & 50.78 {\stdfont $\pm$ .61} & 22.05 {\stdfont $\pm$ .36} & 25.73 {\stdfont $\pm$ .42} \\
    \hline
    \end{tabular} 
}\label{tab:BN_abla}
\end{table}

==> tables/clustering.tex <==

\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\begin{table}[!t]
\caption{Clustering measure. %$\sigma_{btw}$ and $\sigma_{wth}$ for PR have unit of $10^{-4}$.
}
\resizebox{\linewidth}{!}{%
\begin{tabular}{c|c|cccccc}
    \hline
    Measure & PR & miniIN(S) & miniIN(T) & CropDisease & EuroSAT & ISIC & ChestX \\
    \hline
    \multirow{2}{*}{$\sigma_{btw}(\uparrow)$} & \xmark & 2.2894 & 1.8915 & 1.9684 & 1.1410 & 0.6841 & 0.3532 \\
    % & body & 80.96 & 68.94 & 67.27 & 88.88 & 42.20 & 11.40 \\ 
    & \cmark & 0.1008 & 0.1126 & 0.1056 & 0.1595 & 0.0595 & 0.0196 \\ 
    \hline
    \multirow{2}{*}{$\sigma_{wth}(\downarrow)$} & \xmark & 3.3219 & 3.2103 & 2.1576 & 1.1408 & 1.5218 & 1.6643 \\
    % & body & 84.94 & 86.68 & 71.71 & 82.21 & 88.22 & 63.70 \\
    & \cmark & 0.1553 & 0.1551 & 0.1003 & 0.1064 & 0.1130 & 0.0870 \\ 
    \hline
    \multirow{2}{*}{$\text{CM} (\uparrow)$} & \xmark & 0.6892 & 0.5892 & 0.9123 & 1.0002 & 0.4495 & 0.2122 \\
    % & body & \bf 0.9531 & \bf 0.7953 & \bf 0.9381 & \bf 1.0811 & \bf 0.4783 & 0.1790 \\
    & \cmark & \bf 0.7006 & \bf 0.7260 & \bf 1.0528 & \bf 1.4991 & \bf 0.5265 & \bf 0.2253 \\ 
    % \hline\hline
    % \multirow{2}{*}{$\sigma_{btw}(\uparrow)$} & \xmark & 0.2320 & 0.1661 & 0.2319 & 0.4513 & 0.1156 & 0.0138 \\
    % % & body & 0.1762 & 0.1306 & 0.1282 & 0.2211 & 0.0527 & 0.0040 \\   
    % & \cmark & 0.3745 & 0.3972 & 0.3494 & 0.7746 & 0.1138 & 0.0128 \\ 
    % \hline
    % \multirow{2}{*}{$\sigma_{wth}(\downarrow)$} & \xmark & 0.4894 & 0.5072 & 0.2814 & 0.4047 & 0.4924 & 0.3038 \\
    % % & body & 0.1894 & 0.2008 & 0.1486 & 0.1795 & 0.2183 & 0.1258 \\
    % & \cmark & 0.7537 & 0.7447 & 0.2990 & 0.3581 & 0.4044 & 0.2382 \\ 
    % \hline
    % \multirow{2}{*}{$\text{ICC} (\uparrow)$} & \xmark & 0.4740 & 0.3275 & 0.8241 & 1.1151 & 0.2348 & 0.0454 \\
    % % & body & \bf 0.9303 & \bf 0.6504 & \bf 0.8627 & \bf 1.2318 & \bf 0.2414 & 0.0318 \\    
    % & \cmark & \bf 0.4967 &  \bf 0.5333 & \bf 1.1684 & \bf 2.1633 & \bf 0.2815 & \bf 0.0538 \\ 
    \hline
\end{tabular}
}\label{tab:clustering}
\end{table}

==> tables/comparison.tex <==

% \begin{table*}[t]
% \centering
% \caption{Test accuracy over 600 tasks on miniImageNet $\rightarrow$ \{miniImageNet, BSCD-FSL\}. ResNet10 is used and mean and 95\% confidence interval are reported. $^{*}$ denotes the results from \cite{phoo2021selftraining}, where unlabeled data is not used for pre-training. $^{\dagger}$ denotes the results from \cite{phoo2021selftraining}, where 20\% of unlabeled dataset is used for pre-training and 80\% of that is used for evaluation. $^{\ddagger}$ denotes the results from \cite{islam2021dynamic}, similar to \cite{phoo2021selftraining}; however, the splits are different for random sampling. We follow the splits of \cite{phoo2021selftraining} for 80\% evaluation of test dataset. All of our (re-)implementations (Ours) except for `Classifier Transfer' fine-tune the entire network. For ours, \{Conv2, BN2, ShortcutConv, ShortcutBN\} in the last block ($B_4$) are reinitialized.}
% \addtolength{\tabcolsep}{-4pt}
% \resizebox{0.9\textwidth}{!}{%
% \begin{tabular}{c|cc|cc|cc|cc|cc}
%     \hline
%     Source dataset & \multicolumn{10}{c}{miniImageNet} \\
%     \hline
%     \multirow{2}{*}{Target dataset} & \multicolumn{2}{c|}{miniImageNet} & \multicolumn{2}{c|}{CropDisease} & \multicolumn{2}{c|}{EuroSAT} & \multicolumn{2}{c|}{ISIC} & \multicolumn{2}{c}{ChestX} \\
%     & $k=1$ & $k=5$ & $k=1$ & $k=5$ & $k=1$ & $k=5$ & $k=1$ & $k=5$ & $k=1$ & $k=5$ \\
%     \hline \hline
%     \multicolumn{11}{l}{All of target data is used for evaluation.} \\
%     \hline 
%     MAML$^{*}$ & - & - & - & 78.05{\stdfont$\pm$.68} & - & 71.70{\stdfont$\pm$.72} & - & 40.13{\stdfont$\pm$.58} & - & 23.48{\stdfont$\pm$.96} \\
%     ProtoNet$^{*}$ & - & - & - & 79.72{\stdfont$\pm$.67} & - & 73.29{\stdfont$\pm$.71} & - & 39.57{\stdfont$\pm$.57} & - & 24.05{\stdfont$\pm$1.01} \\
%     ProtoNet+FWT$^{*}$ & - & - & - & 72.72{\stdfont$\pm$.70} & - & 67.34{\stdfont$\pm$.76} & - & 38.87{\stdfont$\pm$.52} & - & 23.77{\stdfont$\pm$.42} \\
%     MetaOptNet$^{*}$ & - & - & - & 68.41{\stdfont$\pm$.73} & - & 64.44{\stdfont$\pm$.73} & - & 36.28{\stdfont$\pm$.50} & - & 22.53{\stdfont$\pm$.91} \\
%     Classifier Transfer$^{*}$ & - & - & - & 87.48{\stdfont$\pm$.58} & - & 75.69{\stdfont$\pm$.66} & - & 43.56{\stdfont$\pm$.60} & - & 25.35{\stdfont$\pm$.96} \\
%     Transfer$^{*}$ & - & - & - & 89.25{\stdfont$\pm$.51} & - & 79.08{\stdfont$\pm$.61} & - & 48.11{\stdfont$\pm$.64} & - & 25.97{\stdfont$\pm$.41} \\
%     Classifier Transfer (Re.)    & \textbf{52.32{\stdfont$\pm$.80}} & \textbf{75.67{\stdfont$\pm$.61}} & 65.73{\stdfont$\pm$.87} & 88.68{\stdfont$\pm$.53} & 54.35{\stdfont$\pm$.92} & 75.96{\stdfont$\pm$.67} & 30.42{\stdfont$\pm$.54} & 42.97{\stdfont$\pm$.56} & 22.17{\stdfont$\pm$.37} & 25.80{\stdfont$\pm$.43} \\
%     Transfer (Re.)     & 44.83{\stdfont$\pm$.75} & 73.88{\stdfont$\pm$.64} & 57.57{\stdfont$\pm$.90} & 88.04{\stdfont$\pm$.56} & 51.54{\stdfont$\pm$.85} & 79.33{\stdfont$\pm$.62} & 32.31{\stdfont$\pm$.55} & 49.67{\stdfont$\pm$.60} & 21.82{\stdfont$\pm$.35} & 26.10{\stdfont$\pm$.44} \\
%     Transfer+RR (Ours) & 48.79{\stdfont$\pm$.78} & 70.71{\stdfont$\pm$.67} & 68.83{\stdfont$\pm$.84} & 90.89{\stdfont$\pm$.49} & 62.77{\stdfont$\pm$.82} & 82.24{\stdfont$\pm$.57} & 33.21{\stdfont$\pm$.59} & 49.59{\stdfont$\pm$.63} & 22.82{\stdfont$\pm$.41} & 26.60{\stdfont$\pm$.42} \\
%     % Transfer+RR (Ours) & 51.44{\stdfont$\pm$.79} & 74.81{\stdfont$\pm$.61} & \textbf{72.04{\stdfont$\pm$.84}} & \textbf{91.87{\stdfont$\pm$.46}} & \textbf{67.50{\stdfont$\pm$.84}} & \textbf{83.75{\stdfont$\pm$.58}} & \textbf{34.44{\stdfont$\pm$.64}} & \textbf{51.03{\stdfont$\pm$.61}} & \textbf{22.44{\stdfont$\pm$.40}} & \textbf{26.86{\stdfont$\pm$.41}} \\
%     \hline \hline
    
%     \multicolumn{11}{l}{80\% of target data is used for evaluation. 20\% of that is not used or used for pre-training as unlabeled data.} \\
%     \hline
%     Classifier Transfer$^{\dagger}$ & \textbf{54.18{\stdfont$\pm$.79}} & \textbf{76.20{\stdfont$\pm$.64}} & 69.97{\stdfont$\pm$.85} & 90.16{\stdfont$\pm$.49} & 60.73{\stdfont$\pm$.86} & 80.30{\stdfont$\pm$.64} & 30.71{\stdfont$\pm$.59} & 43.08{\stdfont$\pm$.57} & \textbf{22.71{\stdfont$\pm$.40}} & \textbf{26.71{\stdfont$\pm$.46}} \\
%     Classifier Transfer (Re.)    & 51.90{\stdfont$\pm$.77} & 74.66{\stdfont$\pm$.61} & 65.41{\stdfont$\pm$.88} & 89.02{\stdfont$\pm$.54} & 53.72{\stdfont$\pm$.86} & 74.73{\stdfont$\pm$.63} & 30.15{\stdfont$\pm$.55} & 42.53{\stdfont$\pm$.53} & 22.41{\stdfont$\pm$.37} & 25.66{\stdfont$\pm$.42} \\
%     Transfer (Re.)    & 44.62{\stdfont$\pm$.77} & 73.74{\stdfont$\pm$.65} & 59.28{\stdfont$\pm$.87} & 88.77{\stdfont$\pm$.55} & 52.48{\stdfont$\pm$.80} & 78.83{\stdfont$\pm$.61} &31.33{\stdfont$\pm$.56} &49.23{\stdfont$\pm$.64} & 21.86{\stdfont$\pm$.33} & 25.88{\stdfont$\pm$.41} \\
%     Transfer+RR (Ours) & 47.52{\stdfont$\pm$.83} & 69.85{\stdfont$\pm$.67} & 67.68{\stdfont$\pm$.88} & 90.76{\stdfont$\pm$.52} & 63.02{\stdfont$\pm$.85} & 82.02{\stdfont$\pm$.60} & 32.82{\stdfont$\pm$.63} & 49.26{\stdfont$\pm$.63} & 22.52{\stdfont$\pm$.41} & 26.93{\stdfont$\pm$.41} \\
%     \hline
%     STARTUP$^{\dagger}$ \cite{phoo2021selftraining}          & 54.20{\stdfont$\pm$.81} & 76.48{\stdfont$\pm$.63} & 75.93{\stdfont$\pm$.80} & 93.02{\stdfont$\pm$.45} & 63.88{\stdfont$\pm$.84} & 82.29{\stdfont$\pm$.60} & 32.66{\stdfont$\pm$.60} & 47.22{\stdfont$\pm$.61} & 23.09{\stdfont$\pm$.43} & 26.94{\stdfont$\pm$.44} \\
%     Dynamic Distillation$^{\ddagger}$ \cite{islam2021dynamic} & 53.71{\stdfont$\pm$.83} & 76.02{\stdfont$\pm$.61} & 82.14{\stdfont$\pm$.78} & 95.54{\stdfont$\pm$.38} & 73.14{\stdfont$\pm$.84} & 89.07{\stdfont$\pm$.47} & 34.66{\stdfont$\pm$.58} & 49.36{\stdfont$\pm$.59} & 23.38{\stdfont$\pm$.43} & 28.31{\stdfont$\pm$.46} \\
%     Transfer+RR+SimCLR (Ours) & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} \\
%     \hline
%     \end{tabular} 
% }\label{tab:mini_comparison}
% \end{table*}



% \begin{table*}[t]
% \centering
% \caption{Test accuracy over 600 tasks on tieredImageNet $\rightarrow$ \{tieredImageNet, BSCD-FSL\}. ResNet12 is used and mean and 95\% confidence interval are reported. For ours, \{Conv2, BN2, ShortcutConv, ShortcutBN\} in the last block ($B_4$) are reinitialized.}
% \addtolength{\tabcolsep}{-4pt}
% \resizebox{0.9\textwidth}{!}{%
% \begin{tabular}{c|cc|cc|cc|cc|cc}
%     \hline
%     Source dataset & \multicolumn{10}{c}{tieredImageNet} \\
%     \hline
%     \multirow{2}{*}{Target dataset} & \multicolumn{2}{c|}{tieredImageNet} & \multicolumn{2}{c|}{CropDisease} & \multicolumn{2}{c|}{EuroSAT} & \multicolumn{2}{c|}{ISIC} & \multicolumn{2}{c}{ChestX} \\
%     & $k=1$ & $k=5$ & $k=1$ & $k=5$ & $k=1$ & $k=5$ & $k=1$ & $k=5$ & $k=1$ & $k=5$ \\
%     \hline \hline
%     \multicolumn{11}{l}{All of target data is used for evaluation.} \\
%     \hline 
%     Classifier Transfer (Re.)    & 58.01{\stdfont$\pm$.85} & 79.46{\stdfont$\pm$.68} & 64.35{\stdfont$\pm$.86} & 86.74{\stdfont$\pm$.52} & 56.64{\stdfont$\pm$.91} & 74.66{\stdfont$\pm$.69} & 32.11{\stdfont$\pm$.58} & 43.58{\stdfont$\pm$.58} & 22.12{\stdfont$\pm$.41} & 25.23{\stdfont$\pm$.43} \\
%     Transfer (Re.)    & 49.49{\stdfont$\pm$.78} & 75.70{\stdfont$\pm$.70} & 58.38{\stdfont$\pm$.83} & 86.90{\stdfont$\pm$.57} & 49.00{\stdfont$\pm$.77} & 74.91{\stdfont$\pm$.64} & 32.11{\stdfont$\pm$.56} & 48.58{\stdfont$\pm$.60} & 22.00{\stdfont$\pm$.37} & 24.70{\stdfont$\pm$.40} \\
%     Transfer+RR (Ours)    & 46.11{\stdfont$\pm$.87} & 71.56{\stdfont$\pm$.82} & 64.83{\stdfont$\pm$.98} & 90.33{\stdfont$\pm$.56} & 54.18{\stdfont$\pm$.78} & 76.77{\stdfont$\pm$.66} & 31.66{\stdfont$\pm$.57} & 47.48{\stdfont$\pm$.60} & 21.88{\stdfont$\pm$.37} & 25.65{\stdfont$\pm$.43} \\
%     \hline \hline
%     \multicolumn{11}{l}{80\% of target data is used for evaluation. 20\% of that is not used or used for pre-training as unlabeled data.} \\
%     \hline
%     Classifier Transfer (Re.)    & 57.45{\stdfont$\pm$.85} & 80.01{\stdfont$\pm$.67} & 64.23{\stdfont$\pm$.83} & 86.69{\stdfont$\pm$.55} & 57.25{\stdfont$\pm$.93} & 74.09{\stdfont$\pm$.70} & 31.32{\stdfont$\pm$.58} & 43.69{\stdfont$\pm$.58} & 22.59{\stdfont$\pm$.41} & 25.31{\stdfont$\pm$.44} \\
%     Transfer (Re.)    & 49.40{\stdfont$\pm$.82} & 75.97{\stdfont$\pm$.71} & 58.84{\stdfont$\pm$.82} & 87.07{\stdfont$\pm$.56} & 49.27{\stdfont$\pm$.80} & 74.73{\stdfont$\pm$.64} & 31.90{\stdfont$\pm$.55} & 48.35{\stdfont$\pm$.58} & 21.58{\stdfont$\pm$.38} & 24.61{\stdfont$\pm$.42} \\
%     Transfer+RR (Ours) & 45.67{\stdfont$\pm$.81} & 72.78{\stdfont$\pm$.77} & 64.59{\stdfont$\pm$.01} & 90.27{\stdfont$\pm$.56} & 53.24{\stdfont$\pm$.81} & 77.16{\stdfont$\pm$.67} & 31.47{\stdfont$\pm$.59} & 47.00{\stdfont$\pm$.60} & 21.89{\stdfont$\pm$.37} & 25.97{\stdfont$\pm$.40} \\
%     \hline
%     STARTUP (Re.) \cite{phoo2021selftraining}          & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} \\
%     Dynamic Distillation (Re.) \cite{islam2021dynamic} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} \\
%     Transfer+RR+SimCLR (Ours) & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} \\
%     \hline
%     \end{tabular} 
% }\label{tab:tiered_comparison}
% \end{table*}

% \begin{table*}[t]
% \centering
% \caption{Test accuracy over 600 tasks on ImageNet $\rightarrow$ BSCD-FSL. ResNet18 is used and mean and 95\% confidence interval are reported. For ours, \{Conv2, BN2, ShortcutConv, ShortcutBN\} in the last block ($B_4$) are reinitialized.}
% \addtolength{\tabcolsep}{-4pt}
% \resizebox{0.9\textwidth}{!}{%
% \begin{tabular}{c|cc|cc|cc|cc}
%     \hline
%     Source dataset & \multicolumn{8}{c}{ImageNet} \\
%     \hline
%     \multirow{2}{*}{Target dataset} & \multicolumn{2}{c|}{CropDisease} & \multicolumn{2}{c|}{EuroSAT} & \multicolumn{2}{c|}{ISIC} & \multicolumn{2}{c}{ChestX} \\
%     & $k=1$ & $k=5$ & $k=1$ & $k=5$ & $k=1$ & $k=5$ & $k=1$ & $k=5$ \\
%     \hline \hline
%     \multicolumn{9}{l}{All of target data is used for evaluation.} \\
%     \hline 
%     Classifier Transfer (Re.)    & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} \\
%     Transfer (Re.)    & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} \\
%     Transfer+RR (Ours) & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} \\
%     \hline \hline
%     \multicolumn{9}{l}{80\% of target data is used for evaluation. 20\% of that is not used or used for pre-training as unlabeled data.} \\
%     \hline
%     Classifier Transfer$^{\dagger}$ & 74.17{\stdfont$\pm$.82} & 92.46{\stdfont$\pm$.42} & 66.08{\stdfont$\pm$.81} & 85.58{\stdfont$\pm$.48} & 30.27{\stdfont$\pm$.51} & 43.88{\stdfont$\pm$.56} & 21.97{\stdfont$\pm$.39} & 25.85{\stdfont$\pm$.41} \\
%     Classifier Transfer (Re.)    & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} \\
%     Transfer (Re.)    & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} \\
%     Transfer+RR (Ours) & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} \\
%     \hline
%     STARTUP$^{\dagger}$ \cite{phoo2021selftraining}          & 85.10{\stdfont$\pm$.74} & 96.06{\stdfont$\pm$.33} & 73.83{\stdfont$\pm$.77} & 89.70{\stdfont$\pm$.41} & 31.69{\stdfont$\pm$.59} & 46.02{\stdfont$\pm$.59} & 23.03{\stdfont$\pm$.42} & 27.24{\stdfont$\pm$.46} \\
%     Dynamic Distillation$^{\ddagger}$ \cite{islam2021dynamic} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} \\
%     Transfer+RR+SimCLR (Ours)00 & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} \\
%     \hline
%     \end{tabular} 
% }\label{tab:imagenet_comparison}
% \end{table*}

% \begin{table*}[h]
% \centering
% \addtolength{\tabcolsep}{-4pt}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{c|l|c|cc|cc|cc|cc}
%     \hline
%     \multirow{3}{*}{\shortstack{Source Dataset\\(Backbone)}} & \multirow{3}{*}{Methods} & \multirow{3}{*}{ SS } & \multicolumn{8}{c}{Target Dataset} \\
%     \cline{4-11}
%     & & & \multicolumn{2}{c|}{CropDisease} & \multicolumn{2}{c|}{EuroSAT} & \multicolumn{2}{c|}{ISIC} & \multicolumn{2}{c}{ChestX} \\
%     & & & $k=1$ & $k=5$ & $k=1$ & $k=5$ & $k=1$ & $k=5$ & $k=1$ & $k=5$ \\
%     \hline
%     \multirow{6}{*}{\shortstack{miniImageNet\\(ResNet10)}} & Transfer$^{\dagger}$ & & 69.97{\stdfont$\pm$.85} & 90.16{\stdfont$\pm$.49} & 60.73{\stdfont$\pm$.86} & 80.30{\stdfont$\pm$.64} & 30.71{\stdfont$\pm$.59} & 43.08{\stdfont$\pm$.57} & 22.71{\stdfont$\pm$.40} & 26.71{\stdfont$\pm$.46} \\
%     & SimCLR$^{\dagger}$ & \checkmark  & 78.23{\stdfont$\pm$.83} & 92.57{\stdfont$\pm$.48} & 43.52{\stdfont$\pm$.88} & 59.05{\stdfont$\pm$.70} & 26.25{\stdfont$\pm$.53} & 36.09{\stdfont$\pm$.57} & 22.10{\stdfont$\pm$.41} & 25.02{\stdfont$\pm$.42} \\
%     % & Transfer (Re.) & & 65.41{\stdfont$\pm$.88} & 89.02{\stdfont$\pm$.54} & 53.72{\stdfont$\pm$.86} & 74.73{\stdfont$\pm$.63} & 30.15{\stdfont$\pm$.55} & 42.53{\stdfont$\pm$.53} & 22.41{\stdfont$\pm$.37} & 25.66{\stdfont$\pm$.42} \\
%     % & \textcolor{green}{Transfer (Re.)($^{\ddagger}$)} & & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} \\
%     % & Transfer (Re.) & & 59.28{\stdfont$\pm$.87} & 88.77{\stdfont$\pm$.55} & 52.48{\stdfont$\pm$.80} & 78.83{\stdfont$\pm$.61} &31.33{\stdfont$\pm$.56} &49.23{\stdfont$\pm$.64} & 21.86{\stdfont$\pm$.33} & 25.88{\stdfont$\pm$.41} \\
%     % & \textcolor{green}{Transfer+RR (Ours)} & & 67.68{\stdfont$\pm$.88} & 90.76{\stdfont$\pm$.52} & 63.02{\stdfont$\pm$.85} & 82.02{\stdfont$\pm$.60} & 32.82{\stdfont$\pm$.63} & 49.26{\stdfont$\pm$.63} & 22.52{\stdfont$\pm$.41} & 26.93{\stdfont$\pm$.41} \\
%     & Transfer+SimCLR (Baseline)$^{\dagger}$ & \checkmark  & 76.90{\stdfont$\pm$.78} & 92.64{\stdfont$\pm$.44} & 57.18{\stdfont$\pm$.87} & 77.61{\stdfont$\pm$.66} & 32.63{\stdfont$\pm$.63} & 45.96{\stdfont$\pm$.61} & 22.70{\stdfont$\pm$.40} & 26.95{\stdfont$\pm$.45} \\
%     & Transfer+RR+SimCLR (Ours) & \checkmark & \textbf{90.15{\stdfont$\pm$.76}} & \textbf{96.89{\stdfont$\pm$.38}} & \textbf{81.53{\stdfont$\pm$.73}} & \textbf{93.43{\stdfont$\pm$.31}} & \textbf{35.62{\stdfont$\pm$.64}} & \textbf{49.31{\stdfont$\pm$.62}} & 22.23{\stdfont$\pm$.40} & 24.52{\stdfont$\pm$.42} \\
%     & STARTUP$^{\dagger}$ & \checkmark & 75.93{\stdfont$\pm$.80} & 93.02{\stdfont$\pm$.45} & 63.88{\stdfont$\pm$.84} & 82.29{\stdfont$\pm$.60} & 32.66{\stdfont$\pm$.60} & 47.22{\stdfont$\pm$.61} & \textbf{23.09{\stdfont$\pm$.43}} & 26.94{\stdfont$\pm$.44} \\
%     & STARTUP+RR (Ours) & \checkmark & 88.72{\stdfont$\pm$.71} & 96.82{\stdfont$\pm$.33} & 76.59{\stdfont$\pm$.82} & 89.80{\stdfont$\pm$.42} & 37.55{\stdfont$\pm$.65} & 50.14{\stdfont$\pm$.64} & 22.25{\stdfont$\pm$.46} & 26.63{\stdfont$\pm$.43} \\
%     & Dynamic Distillation$^{\ddagger}$ & \checkmark & 82.14{\stdfont$\pm$.78} & 95.54{\stdfont$\pm$.38} & 73.14{\stdfont$\pm$.84} & 89.07{\stdfont$\pm$.47} & 34.66{\stdfont$\pm$.58} & \textbf{49.36{\stdfont$\pm$.59}} & \textbf{23.38{\stdfont$\pm$.43}} & \textbf{28.31{\stdfont$\pm$.46}} \\
%     & Dynamic Distillation+RR (Ours) & \checkmark & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} \\
%     % & T+RR+SS+RR (Ours) & \checkmark & 77.54{\stdfont$\pm$.80} & 93.97{\stdfont$\pm$.44} & 66.95{\stdfont$\pm$.84} & 86.33{\stdfont$\pm$.53} & 34.24{\stdfont$\pm$.64} & 49.60{\stdfont$\pm$.64} & 22.67{\stdfont$\pm$.42} & 27.01{\stdfont$\pm$.42} \\
%     % & \textcolor{green}{Ours + freeze bn} & \checkmark & 85.54{\stdfont$\pm$.80} & 95.97{\stdfont$\pm$.37} & 71.58{\stdfont$\pm$.84} & 90.23{\stdfont$\pm$.42} & 32.13{\stdfont$\pm$.60} & 47.14{\stdfont$\pm$.61} & 21.94{\stdfont$\pm$.39} & 25.88{\stdfont$\pm$.42}  \\
%     \hline
%     \multirow{6}{*}{\shortstack{tieredImageNet\\(ResNet18)}} & Transfer$^{*}$ & & 63.93{\stdfont$\pm$.85} & 85.73{\stdfont$\pm$.60} & 50.62{\stdfont$\pm$.86} & 72.24{\stdfont$\pm$.65} & 32.31{\stdfont$\pm$.60} & \textbf{46.36{\stdfont$\pm$.65}} & 22.49{\stdfont$\pm$.41} & 25.76{\stdfont$\pm$.41} \\
%     & SimCLR$^{*}$ & \checkmark & 87.94{\stdfont$\pm$.74} & 96.50{\stdfont$\pm$.35} & 65.57{\stdfont$\pm$.85} & 85.19{\stdfont$\pm$.50} & 33.92{\stdfont$\pm$.62} & 44.34{\stdfont$\pm$.61} & 21.82{\stdfont$\pm$.41} & 24.42{\stdfont$\pm$.46} \\
%     & Transfer+SimCLR$^{*}$ & \checkmark & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & 68.57{\stdfont$\pm$.81} & 87.64{\stdfont$\pm$.45} & 31.23{\stdfont$\pm$.61} & 41.62{\stdfont$\pm$.55} & 22.41{\stdfont$\pm$.41} & 24.41{\stdfont$\pm$.40} \\
%     & Transfer+RR+SimCLR (Ours) & \checkmark & \textbf{91.18{\stdfont$\pm$.73}} & \textbf{97.25{\stdfont$\pm$.35}} & \textbf{81.69{\stdfont$\pm$.74}} & \textbf{93.43{\stdfont$\pm$.33}} & \textbf{34.17{\stdfont$\pm$.64}} & 46.01{\stdfont$\pm$.56} & 22.20{\stdfont$\pm$.42} & 24.68{\stdfont$\pm$.43} \\
%     & STARTUP$^{\ddagger}$ & \checkmark & 70.09{\stdfont$\pm$.86} & 90.81{\stdfont$\pm$.49} & 64.32{\stdfont$\pm$.87} & 85.19{\stdfont$\pm$.50} & 29.73{\stdfont$\pm$.51} & 43.55{\stdfont$\pm$.56} & 22.10{\stdfont$\pm$.40} & 26.03{\stdfont$\pm$.44} \\
%     & STARTUP+RR (Ours) & \checkmark & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} \\
%     & Dynamic Distillation$^{\ddagger}$ & \checkmark & 84.41{\stdfont$\pm$.75} & 95.90{\stdfont$\pm$.34} & 72.15{\stdfont$\pm$.75} & 89.44{\stdfont$\pm$.42} & \textbf{33.87{\stdfont$\pm$.56}} & \textbf{47.21{\stdfont$\pm$.56}} & 22.70{\stdfont$\pm$.42} & 27.67{\stdfont$\pm$.46} \\
%     & Dynamic Distillation+RR (Ours) & \checkmark & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} \\
%     \hline
%     \multirow{6}{*}{\shortstack{ImageNet\\(ResNet18)}} & Transfer$^{*}$ & & 73.90{\stdfont$\pm$.82} & 92.81{\stdfont$\pm$.45} & 66.14{\stdfont$\pm$.83} & 84.73{\stdfont$\pm$.51} & 31.11{\stdfont$\pm$.55} & 44.10{\stdfont$\pm$.58} & \textbf{22.48{\stdfont$\pm$.39}} & 25.51{\stdfont$\pm$.44} \\
%     % & Transfer (Re.) & & 68.21{\stdfont$\pm$.89} & 91.70{\stdfont$\pm$.49} & 49.75{\stdfont$\pm$.85} & 74.38{\stdfont$\pm$.66} & 31.90{\stdfont$\pm$.54} & 49.71{\stdfont$\pm$.61} & 21.79{\stdfont$\pm$.38} & 25.35{\stdfont$\pm$.41} \\
%     % & RR (Ours) & & 70.42{\stdfont$\pm$.90} & 94.07{\stdfont$\pm$.43} & 50.18{\stdfont$\pm$.82} & 79.56{\stdfont$\pm$.58} & 31.39{\stdfont$\pm$.57} & 49.66{\stdfont$\pm$.57} & 21.67{\stdfont$\pm$.35} & 25.48{\stdfont$\pm$.42} \\
%     & SimCLR$^{*}$ & \checkmark & 88.25{\stdfont$\pm$.75} & 96.33{\stdfont$\pm$.38} & 64.72{\stdfont$\pm$.82} & 84.23{\stdfont$\pm$.52} & 34.06{\stdfont$\pm$.67} & 44.63{\stdfont$\pm$.66} & 22.26{\stdfont$\pm$.41} & 24.43{\stdfont$\pm$.44} \\
%     & Transfer+SimCLR$^{*}$ & \checkmark & 89.85{\stdfont$\pm$.69} & \textbf{97.12{\stdfont$\pm$.33}} & 68.15{\stdfont$\pm$.88} & 86.73{\stdfont$\pm$.47} & 34.28{\stdfont$\pm$.63} & 43.92{\stdfont$\pm$.63} & 21.98{\stdfont$\pm$.40} & 24.54{\stdfont$\pm$.44} \\
%     & Transfer+RR+SimCLR (Ours) & \checkmark & \textbf{91.13{\stdfont$\pm$.73}} & \textbf{96.95{\stdfont$\pm$.38}} & \textbf{84.92{\stdfont$\pm$.67}} & \textbf{94.58{\stdfont$\pm$.29}} & \textbf{36.80{\stdfont$\pm$.68}} & \textbf{48.63{\stdfont$\pm$.62}} & 21.70{\stdfont$\pm$.42} & 24.78{\stdfont$\pm$.43} \\
%     & STARTUP$^{\dagger}$ & \checkmark & 85.10{\stdfont$\pm$.74} & 96.06{\stdfont$\pm$.33} & 73.83{\stdfont$\pm$.77} & 89.70{\stdfont$\pm$.41} & 31.69{\stdfont$\pm$.59} & 46.02{\stdfont$\pm$.59} & \textbf{23.03{\stdfont$\pm$.42}} & \textbf{27.24{\stdfont$\pm$.46}} \\
%     & STARTUP+RR (Ours) & \checkmark & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} \\
%     & Dynamic Distillation (Re.) & \checkmark & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} \\
%     & Dynamic Distillation+RR (Ours) & \checkmark & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} \\
%     \hline
%     \end{tabular} 
% }
% \caption{\textbf{5way-$k$shot test accuracy over 600 tasks on \{miniImageNet, tieredImageNet, ImageNet\} $\rightarrow$ \{BSCD-FSL\}. All methods are evaluated using 80\% of the original test dataset.} ResNet10 is pre-trained on miniImageNet and ResNet18 is pre-trained on tieredImageNet and ImageNet. $^{\dagger}$ and $^{\ddagger}$ denote the results from \cite{phoo2021selftraining} and \cite{islam2021dynamic}, respectively. $^{*}$ indicates our re-implementation. SS indicates the algorithms that use 20\% of the original test dataset as unlabeled target data in a self-supervised manner. Note that $^{\dagger}$ and $^{\ddagger}$ use different target data splits, of which we follow $^{\dagger}$. For STAR (Ours), topmost layers (\ie, \{Conv2, BN2, ShortcutConv, ShortcutBN\} (ResNet10) and \{Block2.Conv2, Block2.BN2\} (ResNet18)) in the last stage are re-randomized and then self-trained using the SimCLR loss. Mean and 95\% confidence interval are reported. Bolded values are top accuracies that are not different at significant level 0.05.}
% \label{tab:BSCD_comparison}
% \end{table*}


\begin{table*}[h]
\centering
\addtolength{\tabcolsep}{-4pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|l|cc|cc|cc|cc}
    \hline
    \multirow{3}{*}{Methods} & \multirow{3}{*}{Source Dataset} & \multicolumn{8}{c}{Target Dataset} \\
    \cline{3-10}
    & & \multicolumn{2}{c|}{CropDisease} & \multicolumn{2}{c|}{EuroSAT} & \multicolumn{2}{c|}{ISIC} & \multicolumn{2}{c}{ChestX} \\
    & & $k=1$ & $k=5$ & $k=1$ & $k=5$ & $k=1$ & $k=5$ & $k=1$ & $k=5$ \\
    \hline
    \multirow{3}{*}{No pre-train} & miniImagetNet& 53.53{\stdfont$\pm$.92} & 87.53{\stdfont$\pm$.57} & 38.79{\stdfont$\pm$.77} & 79.66{\stdfont$\pm$.79} & 26.23{\stdfont$\pm$.55} & 65.95{\stdfont$\pm$1.06} & 20.92{\stdfont$\pm$.38} & 20.78{\stdfont$\pm$.39} \\
    & tieredImageNet & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} \\
    & ImageNet & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} \\
    \hline
    \multirow{3}{*}{Transfer} & miniImagetNet$^{\dagger}$ & 69.97{\stdfont$\pm$.85} & 90.16{\stdfont$\pm$.49} & 60.73{\stdfont$\pm$.86} & 80.30{\stdfont$\pm$.64} & 30.71{\stdfont$\pm$.59} & 43.08{\stdfont$\pm$.57} & 22.71{\stdfont$\pm$.40} & 26.71{\stdfont$\pm$.46} \\
    & tieredImageNet & 63.93{\stdfont$\pm$.85} & 85.73{\stdfont$\pm$.60} & 50.62{\stdfont$\pm$.86} & 72.24{\stdfont$\pm$.65} & 32.31{\stdfont$\pm$.60} & \textbf{46.36{\stdfont$\pm$.65}} & 22.49{\stdfont$\pm$.41} & 25.76{\stdfont$\pm$.41} \\
    & ImageNet & 74.18{\stdfont$\pm$.82} & 92.81{\stdfont$\pm$.45} & 66.14{\stdfont$\pm$.83} & 84.73{\stdfont$\pm$.51} & 31.11{\stdfont$\pm$.55} & 44.10{\stdfont$\pm$.58} & \textbf{22.48{\stdfont$\pm$.39}} & 25.51{\stdfont$\pm$.44} \\
    \hline
    % \multirow{3}{*}{SimCLR} & miniImagetNet$^{\dagger}$ & 78.23{\stdfont$\pm$.83} & 92.57{\stdfont$\pm$.48} & 43.52{\stdfont$\pm$.88} & 59.05{\stdfont$\pm$.70} & 26.25{\stdfont$\pm$.53} & 36.09{\stdfont$\pm$.57} & 22.10{\stdfont$\pm$.41} & 25.02{\stdfont$\pm$.42} \\
    % & tieredImageNet & 87.94{\stdfont$\pm$.74} & 96.50{\stdfont$\pm$.35} & 65.57{\stdfont$\pm$.85} & 85.19{\stdfont$\pm$.50} & 33.92{\stdfont$\pm$.62} & 44.34{\stdfont$\pm$.61} & 21.82{\stdfont$\pm$.41} & 24.42{\stdfont$\pm$.46} \\
    % & ImageNet & 88.25{\stdfont$\pm$.75} & 96.33{\stdfont$\pm$.38} & 64.72{\stdfont$\pm$.82} & 84.23{\stdfont$\pm$.52} & 34.06{\stdfont$\pm$.67} & 44.63{\stdfont$\pm$.66} & 22.26{\stdfont$\pm$.41} & 24.43{\stdfont$\pm$.44} \\
    % \hline
    \multirow{3}{*}{TranSimCLR} & miniImagetNet$^{\dagger}$ & 76.90{\stdfont$\pm$.78} & 92.64{\stdfont$\pm$.44} & 57.18{\stdfont$\pm$.87} & 77.61{\stdfont$\pm$.66} & 32.63{\stdfont$\pm$.63} & 45.96{\stdfont$\pm$.61} & 22.70{\stdfont$\pm$.40} & 26.95{\stdfont$\pm$.45} \\
    & tieredImageNet & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & 68.57{\stdfont$\pm$.81} & 87.64{\stdfont$\pm$.45} & 31.23{\stdfont$\pm$.61} & 41.62{\stdfont$\pm$.55} & 22.41{\stdfont$\pm$.41} & 24.41{\stdfont$\pm$.40} \\
    & ImageNet & 89.85{\stdfont$\pm$.69} & \textbf{97.12{\stdfont$\pm$.33}} & 68.15{\stdfont$\pm$.88} & 86.73{\stdfont$\pm$.47} & 34.28{\stdfont$\pm$.63} & 43.92{\stdfont$\pm$.63} & 21.98{\stdfont$\pm$.40} & 24.54{\stdfont$\pm$.44} \\
    \hline
    \multirow{3}{*}{\makecell[l]{TranSimCLR \\+ RESET}} & miniImagetNet & \textbf{90.15{\stdfont$\pm$.76}} & \textbf{96.89{\stdfont$\pm$.38}} & \textbf{81.53{\stdfont$\pm$.73}} & \textbf{93.43{\stdfont$\pm$.31}} & \textbf{35.62{\stdfont$\pm$.64}} & \textbf{49.31{\stdfont$\pm$.62}} & 22.23{\stdfont$\pm$.40} & 24.52{\stdfont$\pm$.42} \\
    & tieredImageNet & \textbf{91.18{\stdfont$\pm$.73}} & \textbf{97.25{\stdfont$\pm$.35}} & \textbf{81.69{\stdfont$\pm$.74}} & \textbf{93.43{\stdfont$\pm$.33}} & \textbf{34.17{\stdfont$\pm$.64}} & 46.01{\stdfont$\pm$.56} & 22.20{\stdfont$\pm$.42} & 24.68{\stdfont$\pm$.43} \\
    & ImageNet & \textbf{91.13{\stdfont$\pm$.73}} & \textbf{96.95{\stdfont$\pm$.38}} & \textbf{84.92{\stdfont$\pm$.67}} & \textbf{94.58{\stdfont$\pm$.29}} & \textbf{36.80{\stdfont$\pm$.68}} & \textbf{48.63{\stdfont$\pm$.62}} & 21.70{\stdfont$\pm$.42} & 24.78{\stdfont$\pm$.43} \\
    \hline
    \multirow{3}{*}{STARTUP \cite{phoo2021selftraining}} & miniImagetNet$^{\dagger}$ & 75.93{\stdfont$\pm$.80} & 93.02{\stdfont$\pm$.45} & 63.88{\stdfont$\pm$.84} & 82.29{\stdfont$\pm$.60} & 32.66{\stdfont$\pm$.60} & 47.22{\stdfont$\pm$.61} & \textbf{23.09{\stdfont$\pm$.43}} & 26.94{\stdfont$\pm$.44} \\
    & tieredImageNet$^{\ddagger}$ & 70.09{\stdfont$\pm$.86} & 90.81{\stdfont$\pm$.49} & 64.32{\stdfont$\pm$.87} & 85.19{\stdfont$\pm$.50} & 29.73{\stdfont$\pm$.51} & 43.55{\stdfont$\pm$.56} & 22.10{\stdfont$\pm$.40} & 26.03{\stdfont$\pm$.44} \\
    & ImageNet$^{\dagger}$ & 85.10{\stdfont$\pm$.74} & 96.06{\stdfont$\pm$.33} & 73.83{\stdfont$\pm$.77} & 89.70{\stdfont$\pm$.41} & 31.69{\stdfont$\pm$.59} & 46.02{\stdfont$\pm$.59} & \textbf{23.03{\stdfont$\pm$.42}} & \textbf{27.24{\stdfont$\pm$.46}} \\
    \hline
    \multirow{3}{*}{STARTUP + Strong \cite{phoo2021selftraining}} & miniImagetNet$^{\dagger}$ & 86.49{\stdfont$\pm$.77} & 96.02{\stdfont$\pm$.37} & 74.52{\stdfont$\pm$.83} & 89.30{\stdfont$\pm$.43} & 36.01{\stdfont$\pm$.65} & 48.34{\stdfont$\pm$.64} & 22.48{\stdfont$\pm$.46} & 26.30{\stdfont$\pm$.44} \\
    & tieredImageNet & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} \\
    & ImageNet & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} \\
    \hline
    \multirow{3}{*}{\makecell[l]{STARTUP \cite{phoo2021selftraining}\\+ RESET}} & miniImagetNet & 88.72{\stdfont$\pm$.71} & 96.82{\stdfont$\pm$.33} & 76.59{\stdfont$\pm$.82} & 89.80{\stdfont$\pm$.42} & 37.55{\stdfont$\pm$.65} & 50.14{\stdfont$\pm$.64} & 22.25{\stdfont$\pm$.46} & 26.63{\stdfont$\pm$.43} \\
    & tieredImageNet & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} \\
    & ImageNet & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} \\
    \hline
    \multirow{3}{*}{Dynamic Distillation \cite{islam2021dynamic}} & miniImagetNet$^{\ddagger}$ & 82.14{\stdfont$\pm$.78} & 95.54{\stdfont$\pm$.38} & 73.14{\stdfont$\pm$.84} & 89.07{\stdfont$\pm$.47} & 34.66{\stdfont$\pm$.58} & \textbf{49.36{\stdfont$\pm$.59}} & \textbf{23.38{\stdfont$\pm$.43}} & \textbf{28.31{\stdfont$\pm$.46}} \\
    & tieredImageNet$^{\ddagger}$ & 84.41{\stdfont$\pm$.75} & 95.90{\stdfont$\pm$.34} & 72.15{\stdfont$\pm$.75} & 89.44{\stdfont$\pm$.42} & \textbf{33.87{\stdfont$\pm$.56}} & \textbf{47.21{\stdfont$\pm$.56}} & 22.70{\stdfont$\pm$.42} & 27.67{\stdfont$\pm$.46} \\
    & ImageNet & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} \\
    \hline
    \multirow{3}{*}{\makecell[l]{Dynamic Distillation \cite{islam2021dynamic}\\+ RESET}} & miniImagetNet & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} \\
    & tieredImageNet & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} \\
    & ImageNet & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} \\
    \hline
    \end{tabular} 
}
\caption{\textbf{5way-$k$shot test accuracy over 600 tasks on \{miniImageNet, tieredImageNet, ImageNet\} $\rightarrow$ \{BSCD-FSL\}. All methods are evaluated using 80\% of the original test dataset.} ResNet10 is pre-trained on miniImageNet and ResNet18 is pre-trained on tieredImageNet and ImageNet. $^{\dagger}$ and $^{\ddagger}$ denote the results from \cite{phoo2021selftraining} and \cite{islam2021dynamic}, respectively. Others are (re-)implemented. SS indicates the algorithms that use 20\% of the original test dataset as unlabeled target data in a self-supervised manner. Note that $^{\dagger}$ and $^{\ddagger}$ use different target data splits, of which we follow $^{\dagger}$. For STAR (Ours), topmost layers (\ie, \{Conv2, BN2, ShortcutConv, ShortcutBN\} (ResNet10) and \{Block2.Conv2, Block2.BN2\} (ResNet18)) in the last stage are re-randomized and then self-trained using the SimCLR loss. Mean and 95\% confidence interval are reported. Bolded values are top accuracies that are not different at significant level 0.05.}
\label{tab:BSCD_comparison}
\end{table*}

==> tables/comparison_only_RR_2050.tex <==

\begin{table}[h]
\centering
\addtolength{\tabcolsep}{-4pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|l|cc|cc}
    \hline
    \multirow{3}{*}{Source dataset} & \multirow{3}{*}{Methods} & \multicolumn{4}{c}{Target dataset} \\
    \cline{3-6}
    & & $k=20$ & $k=50$ & $k=20$ & $k=50$ \\
    \cline{3-6}
    & & \multicolumn{2}{c|}{CropDisease} & \multicolumn{2}{c}{EuroSAT} \\
    \hline
    \multirow{2}{*}{\shortstack{miniImageNet}} & Transfer (Re.)    &  93.96{\stdfont$\pm$.35} & 95.33{\stdfont$\pm$.31} & 83.90{\stdfont$\pm$.55} & 85.76{\stdfont$\pm$.47} \\
    & Transfer+RR (Ours) & 93.52{\stdfont$\pm$.41} & 94.64{\stdfont$\pm$.34} & 84.21{\stdfont$\pm$.53} & 85.89{\stdfont$\pm$.48} \\
    \cline{2-6}
    \multirow{2}{*}{\shortstack{tieredImageNet}} & Transfer (Re.) & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} \\
    & Transfer+RR (Ours) & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} \\
    \cline{2-6}
    \multirow{2}{*}{\shortstack{ImageNet}} & Transfer (Re.) & 97.00{\stdfont$\pm$.26} & 98.23{\stdfont$\pm$.18} & 91.81{\stdfont$\pm$.31} & 93.71{\stdfont$\pm$.28} \\
    & Transfer+RR (Ours) & 96.83{\stdfont$\pm$.27} & 98.12{\stdfont$\pm$.19} & 91.69{\stdfont$\pm$.34} & 93.60{\stdfont$\pm$.28} \\
    \hline
    & & \multicolumn{2}{c|}{ISIC} & \multicolumn{2}{c}{ChestX} \\
    \hline
    \multirow{2}{*}{\shortstack{miniImageNet}} & Transfer (Re.)    &  48.21{\stdfont$\pm$.55} & 51.50{\stdfont$\pm$.54} & 28.49{\stdfont$\pm$.41} & 31.31{\stdfont$\pm$.44} \\
    & Transfer+RR (Ours) & 48.72{\stdfont$\pm$.53} & 51.60{\stdfont$\pm$.55} & 28.61{\stdfont$\pm$.43} & 30.72{\stdfont$\pm$.41} \\
    \cline{2-6}
    \multirow{2}{*}{\shortstack{tieredImageNet}} & Transfer (Re.) & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} \\
    & Transfer+RR (Ours) & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} & xx.xx{\stdfont$\pm$.xx} \\
    \cline{2-6}
    \multirow{2}{*}{\shortstack{ImageNet}} & Transfer (Re.) & 54.66{\stdfont$\pm$.58} & 61.36{\stdfont$\pm$.57} & 29.24{\stdfont$\pm$.46} & xx.xx{\stdfont$\pm$.xx} \\
    & Transfer+RR (Ours) & 54.72{\stdfont$\pm$.61} & 60.52{\stdfont$\pm$.55} & 29.32{\stdfont$\pm$.45} & xx.xx{\stdfont$\pm$.xx} \\
    \hline
    \end{tabular} 
}
\caption{\textbf{5way-$k$shot test accuracy over 600 tasks on \{miniImageNet, tieredImageNet, ImageNet\} $\rightarrow$ \{BSCD-FSL\}. All methods are evaluated using 100\% of the original test dataset.} For Transfer+RR (Ours), top layers (\ie, \{Conv2, BN2, ShortcutConv, ShortcutBN\} (ResNet10) and \{Block2.Conv2, Block2.BN2\} (ResNet18)) in the last stage are re-randomized. Mean and 95\% confidence interval are reported.}
\label{tab:BSCD_comparison_all_2050}
\end{table}

==> tables/comparison_only_RR_same.tex <==
\begin{table}[t!]
\small
\centering
\caption{Same-domain 5-way $k$-shot test accuracy over 600 tasks on \{miniImageNet, tieredImageNet\}.}
\label{tab:same_domain_comparison_all}
\addtolength{\tabcolsep}{-3pt}{%
\begin{tabular}{c|cc|cc}
    \toprule
     & \multicolumn{4}{c}{Dataset} \\
    \cmidrule{2-5}
     & \multicolumn{2}{c|}{miniImageNet} & \multicolumn{2}{c}{tieredImageNet} \\
     Methods & $k=1$ & $k=5$ & $k=1$ & $k=5$ \\
    \midrule
    Linear  & \textbf{51.88{\stdfont$\pm$.80}} & \textbf{74.61{\stdfont$\pm$.65}} & \textbf{61.11{\stdfont$\pm$.88}} & \textbf{80.33{\stdfont$\pm$.65}} \\
    Transfer & 44.83{\stdfont$\pm$.75} & 73.88{\stdfont$\pm$.64} & 49.49{\stdfont$\pm$.78} & 75.70{\stdfont$\pm$.70} \\
    ReFine & 49.65{\stdfont$\pm$.75} & 73.84{\stdfont$\pm$.67} & 52.26{\stdfont$\pm$.81} & 75.83{\stdfont$\pm$.69}\\
    \bottomrule
    \end{tabular} 
}
\vspace*{-8pt}
\end{table}

==> tables/comparison_same.tex <==
\begin{table}[h]
\centering
\addtolength{\tabcolsep}{-4pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|c|cc|cc}
    \hline
    \multirow{3}{*}{Methods} & \multirow{3}{*}{ SS } & \multicolumn{4}{c}{Dataset} \\
    \cline{3-6}
     & & \multicolumn{2}{c|}{miniImageNet} & \multicolumn{2}{c}{tieredImageNet} \\
     & & $k=1$ & $k=5$ & $k=1$ & $k=5$ \\
    \hline
    % Transfer$^{\dagger}$ & & 54.18 {\stdfont $\pm$ .79} & 76.20 {\stdfont $\pm$ .64} & 60.73 {\stdfont $\pm$ .86} & 80.30 {\stdfont $\pm$ .64} \\
    Transfer (Re.) & & 51.40{\stdfont $\pm$.78} & 74.80{\stdfont $\pm$.63} & 61.13{\stdfont $\pm$.92} & 80.24{\stdfont $\pm$.69} \\
    % Classifier Transfer (Re.)    & & 51.90 {\stdfont $\pm$ .77} & 74.66 {\stdfont $\pm$ .61} & 53.72 {\stdfont $\pm$ .86} & 74.73 {\stdfont $\pm$ .63} \\
    % Transfer (Re.)    & & 44.62 {\stdfont $\pm$ .77} & 73.74 {\stdfont $\pm$ .65} & 52.48 {\stdfont $\pm$ .80} & 78.83 {\stdfont $\pm$ .61} \\
    % Transfer+RR (Ours) & & 47.52 {\stdfont $\pm$ .83} & 69.85 {\stdfont $\pm$ .67} & 63.02 {\stdfont $\pm$ .85} & 82.02 {\stdfont $\pm$ .60} \\
    SimCLR (Re.) & \checkmark & 54.53{\stdfont $\pm$.96} & 73.40{\stdfont $\pm$.75} & 44.82{\stdfont $\pm$.88} & 60.37{\stdfont $\pm$.84} \\
    Transfer+SimCLR (Re.) & \checkmark & 56.26{\stdfont $\pm$.92} & \textbf{79.26{\stdfont $\pm$.64}} & 45.50{\stdfont $\pm$.86} & 61.75{\stdfont $\pm$.83} \\
    STARTUP$^{\ddagger}$         & \checkmark & 51.68{\stdfont $\pm$.84} & 74.05{\stdfont $\pm$.66} & 60.92{\stdfont $\pm$.96} & 82.11{\stdfont $\pm$.64} \\
    Dynamic Distillation$^{\ddagger}$ & \checkmark & 53.71{\stdfont $\pm$.83} & 76.02{\stdfont $\pm$.61} & 69.00{\stdfont $\pm$.96} & 85.93{\stdfont $\pm$.60} \\
    Transfer+RR+SimCLR (Ours) & \checkmark & \textbf{58.45{\stdfont $\pm$.89}} & \textbf{79.26{\stdfont $\pm$.63}} & 59.22{\stdfont $\pm$1.00} & 75.34{\stdfont $\pm$.79} \\
    \hline
    \end{tabular} 
}
\caption{\textbf{Same-domain 5way-$k$shot test accuracy over 600 tasks on miniImageNet and tieredImageNet, respectively. All methods are evaluated using 80\% of the original test dataset.} The setting is the same as \Cref{tab:BSCD_comparison}.$^\ddagger$ denotes the results from \cite{islam2021dynamic}.}
\label{tab:same_domain_comparison}
\end{table}

==> tables/reinit_scale.tex <==
\begin{table}[ht]
\resizebox{\linewidth}{!}{%
\begin{tabular}{c|c|c|cccc}
    \hline
    Shot & Scale & miniImageNet & CropDisease & EuroSAT & ISIC & ChestX \\
    \hline
    \multirow{5}{*}{1} & 10.0 & 39.74{\stdfont $\pm$.78} & 53.30{\stdfont $\pm$1.01} & 54.46{\stdfont $\pm$.90} & 29.00{\stdfont $\pm$.53} & 21.40{\stdfont $\pm$.31} \\
    & 5.0 & 40.68{\stdfont $\pm$.77} & 55.99{\stdfont $\pm$.95} & 56.15{\stdfont $\pm$.85} & 29.12{\stdfont $\pm$.52} & 21.21{\stdfont $\pm$.32} \\
    & 1.0 & \textbf{48.79{\stdfont $\pm$.78}} & \textbf{68.83{\stdfont $\pm$.84}} & \textbf{62.77{\stdfont $\pm$.82}} & \textbf{33.21{\stdfont $\pm$.59}} & \textbf{22.82{\stdfont $\pm$.41}} \\
    & 0.5 & \textbf{48.14{\stdfont $\pm$.81}} & \textbf{68.46{\stdfont $\pm$.85}} & 60.53{\stdfont $\pm$.82} & 31.28{\stdfont $\pm$.58} & \textbf{22.30{\stdfont $\pm$.38}} \\
    & 0.1 & 44.78{\stdfont $\pm$.79} & 63.84{\stdfont $\pm$.89} & 55.04{\stdfont $\pm$.85} & 30.38{\stdfont $\pm$.54} & 22.11{\stdfont $\pm$.39} \\
    % \cline{2-8}
    % & \multirow{5}{*}{body} & 10.0 & 36.74 $\pm$ 0.77 & 49.35 $\pm$ 1.13  & 56.84 $\pm$ 0.97 & 28.82 $\pm$ 0.54 & 21.15 $\pm$ 0.31 \\
    % & & 5.0 & 38.85 $\pm$ 0.72 & 52.11 $\pm$ 1.04 & 58.71 $\pm$ 0.89 & 29.52 $\pm$ 0.53 & 21.20 $\pm$ 0.32 \\
    % & & 1.0 & 51.44 $\pm$ 0.79 & 72.04 $\pm$ 0.84 & 67.50 $\pm$ 0.84 & \bf 34.44 $\pm$ 0.64 & 22.44 $\pm$ 0.40 \\
    % & & 0.5 & \bf 52.31 $\pm$ 0.85 & \bf 75.46 $\pm$ 0.80 & \bf 67.61 $\pm$ 0.89 & 34.24 $\pm$ 0.64 & \bf 23.34 $\pm$ 0.41 \\
    % & & 0.1 & 49.22 $\pm$ 0.88 & 71.02 $\pm$ 0.87 & 66.08 $\pm$ 0.87 & 33.24 $\pm$ 0.66 & 22.48 $\pm$ 0.41 \\
    \hline
    \multirow{5}{*}{5} & 10.0 & 63.86{\stdfont $\pm$.71} & 86.31{\stdfont $\pm$.58} & 79.23{\stdfont $\pm$.64} & 43.27{\stdfont $\pm$.57} & 24.95{\stdfont $\pm$.39} \\
    & 5.0 & 65.30{\stdfont $\pm$.70} & 87.74{\stdfont $\pm$.57} & 80.51{\stdfont $\pm$.60} & 44.15{\stdfont $\pm$.54} & 25.54{\stdfont $\pm$.43} \\
    & 1.0 & \textbf{70.71{\stdfont $\pm$.67}} & \textbf{90.89{\stdfont $\pm$.49}} & \textbf{82.24{\stdfont $\pm$.57}} & \textbf{49.59{\stdfont $\pm$.63}} & \textbf{26.60{\stdfont $\pm$.42}} \\
    & 0.5 & 67.88{\stdfont $\pm$.72} & \textbf{91.18{\stdfont $\pm$.49}} & 80.84{\stdfont $\pm$.58} & 46.47{\stdfont $\pm$.59} & \textbf{26.82{\stdfont $\pm$.45}} \\
    & 0.1 & 66.40{\stdfont $\pm$.73} & \textbf{90.54{\stdfont $\pm$.48}} & 78.65{\stdfont $\pm$.61} & 46.23{\stdfont $\pm$.61} & \textbf{26.48{\stdfont $\pm$.44}} \\
    % \cline{2-8}
    % & \multirow{5}{*}{body} & 10.0 & 66.03 $\pm$ 0.69 & 87.25 $\pm$ 0.57 & 81.78 $\pm$ 0.61 & 45.81 $\pm$ 0.59 & 24.83 $\pm$ 0.42 \\
    % & & 5.0 & 67.22 $\pm$ 0.71 & 88.76 $\pm$ 0.56 & 82.56 $\pm$ 0.61 & 47.31 $\pm$ 0.60 & 25.71 $\pm$ 0.42 \\
    % & & 1.0 & \bf 74.81 $\pm$ 0.61 & 91.87 $\pm$ 0.46 & \bf 83.75 $\pm$ 0.58 & \bf 51.03 $\pm$ 0.61 & 26.86 $\pm$ 0.41 \\
    % & & 0.5 & 71.30 $\pm$ 0.63 & \bf 93.02 $\pm$ 0.42 & 83.44 $\pm$ 0.59 & 49.95 $\pm$ 0.65 & \bf 27.21 $\pm$ 0.45 \\
    % & & 0.1 & 68.87 $\pm$ 0.69 & 92.41 $\pm$ 0.46 & 82.12 $\pm$ 0.62 & 49.94 $\pm$ 0.60 & 27.03 $\pm$ 0.45 \\
    \hline
\end{tabular}
}
\caption{Analysis on the re-initialization scale of Transfer+PR model.}\label{tab:reinit_scale}
\end{table}


==> tables/subnetworks.tex <==
% \begin{table}[ht]
% \caption{Test accuracy over 600 tasks on miniImageNet $\rightarrow$ \{miniImageNet, BSCD-FSL\} of subnetworks. To evaluate subnetworks, the output of subnetworks is fed into average pooling and a linear classifier. Only the linear classifier is trained. ResNet10 is used and mean and 95\% confidence interval are reported.}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{c|c|c|ccccc}
%     \hline
%     Shot & Subnetwork & Pre-training & miniImageNet & CropDisease & EuroSAT & ISIC & ChestX \\
%     \hline
%     \multirow{8}{*}{1} & \multirow{2}{*}{Block1} & full & 33.79 $\pm$ 0.68 & 46.66 $\pm$ 0.98 & 46.42 $\pm$ 0.82 & 26.77 $\pm$ 0.51 & 20.59 $\pm$ 0.28 \\
%     & & body & 30.89 $\pm$ 0.63 & 41.14 $\pm$ 0.88 & 44.02 $\pm$ 0.83 & 26.06 $\pm$ 0.49 & 20.51 $\pm$ 0.27 \\ \cline{2-8}
%     & \multirow{2}{*}{Block2} & full & 39.31 $\pm$ 0.72 & 57.82 $\pm$ 0.94 & 54.05 $\pm$ 0.86 & 28.01 $\pm$ 0.52 & 20.84 $\pm$ 0.32 \\
%     & & body & 38.89 $\pm$ 0.78 & 49.83 $\pm$ 1.00 & 53.28 $\pm$ 0.83 & 28.38 $\pm$ 0.57 & 20.57 $\pm$ 0.29 \\ \cline{2-8}
%     & \multirow{2}{*}{Block3} & full & 47.28 $\pm$ 0.80 & 65.69 $\pm$ 0.85 & 61.56 $\pm$ 0.90 & 30.07 $\pm$ 0.56 & 22.00 $\pm$ 0.38 \\
%     & & body & 46.17 $\pm$ 0.79 & 62.62 $\pm$ 1.00 & 65.18 $\pm$ 0.83 & 31.49 $\pm$ 0.59 & 21.81 $\pm$ 0.35 \\ \cline{2-8}
%     & \multirow{2}{*}{Block4} & full & 51.88 $\pm$ 0.80 & 66.55 $\pm$ 0.85 & 54.03 $\pm$ 0.87 & 30.71 $\pm$ 0.54 & 22.36 $\pm$ 0.37 \\
%     & & body & 45.52 $\pm$ 0.86 & 50.46 $\pm$ 1.03 & 53.81 $\pm$ 0.94 & 30.71 $\pm$ 0.57 & 21.37 $\pm$ 0.33 \\
%     \hline
%     \multirow{8}{*}{5} & \multirow{2}{*}{Block1} & full & 48.94 $\pm$ 0.75 & 72.82 $\pm$ 0.80 & 64.74 $\pm$ 0.74 & 34.92 $\pm$ 0.53 & 21.90 $\pm$ 0.35 \\
%     & & body & 49.13 $\pm$ 0.78 & 70.80 $\pm$ 0.78 & 66.38 $\pm$ 0.69 & 36.54 $\pm$ 0.51 & 21.94 $\pm$ 0.36 \\ \cline{2-8}
%     & \multirow{2}{*}{Block2} & full & 56.40 $\pm$ 0.75 & 81.61 $\pm$ 0.62 & 73.65 $\pm$ 0.72 & 37.63 $\pm$ 0.51 & 22.65 $\pm$ 0.36 \\
%     & & body & 58.91 $\pm$ 0.76 & 81.77 $\pm$ 0.62 & 76.60 $\pm$ 0.64 & 41.09 $\pm$ 0.56 & 22.92 $\pm$ 0.38 \\ \cline{2-8}
%     & \multirow{2}{*}{Block3} & full & 67.07 $\pm$ 0.70 & 88.19 $\pm$ 0.57 & 80.26 $\pm$ 0.64 & 40.87 $\pm$ 0.54 & 25.25 $\pm$ 0.41 \\
%     & & body & 67.94 $\pm$ 0.72 & 89.39 $\pm$ 0.52 & 83.10 $\pm$ 0.58 & 45.90 $\pm$ 0.57 & 25.08 $\pm$ 0.41 \\ \cline{2-8}
%     & \multirow{2}{*}{Block4} & full & 74.61 $\pm$ 0.65 & 88.73 $\pm$ 0.55 & 75.75 $\pm$ 0.64 & 42.86 $\pm$ 0.54 & 25.60 $\pm$ 0.44 \\
%     & & body & 67.50 $\pm$ 0.77 & 80.27 $\pm$ 0.79 & 76.04 $\pm$ 0.74 & 44.32 $\pm$ 0.61 & 23.92 $\pm$ 0.40 \\
%     \hline
%     \multirow{8}{*}{20} & \multirow{2}{*}{Block1} & full & 57.41 $\pm$ 0.68 & 79.63 $\pm$ 0.69 & 70.51 $\pm$ 0.68 & 41.30 $\pm$ 0.52 & 23.47 $\pm$ 0.36 \\
%     & & body & 58.37 $\pm$ 0.73 & 81.46 $\pm$ 0.62 & 74.41 $\pm$ 0.61 & 44.72 $\pm$ 0.52 & 23.37 $\pm$ 0.39 \\ \cline{2-8}
%     & \multirow{2}{*}{Block2} & full & 66.66 $\pm$ 0.66 & 87.93 $\pm$ 0.52 & 80.13 $\pm$ 0.64 & 44.46 $\pm$ 0.53 & 25.16 $\pm$ 0.37 \\
%     & & body & 67.90 $\pm$ 0.67 & 88.79 $\pm$ 0.49 & 84.40 $\pm$ 0.57 & 50.37 $\pm$ 0.53 & 26.01 $\pm$ 0.41 \\ \cline{2-8}
%     & \multirow{2}{*}{Block3} & full & 76.32 $\pm$ 0.59 & 94.02 $\pm$ 0.37 & 86.54 $\pm$ 0.53 & 48.49 $\pm$ 0.52 & 29.10 $\pm$ 0.42 \\
%     & & body & 77.42 $\pm$ 0.55 & 94.11 $\pm$ 0.37 & 89.20 $\pm$ 0.49 & 55.12 $\pm$ 0.56 & 28.79 $\pm$ 0.42 \\ \cline{2-8}
%     & \multirow{2}{*}{Block4} & full & 83.89 $\pm$ 0.48 & 93.78 $\pm$ 0.40 & 80.27 $\pm$ 0.58 & 49.50 $\pm$ 0.52 & 29.20 $\pm$ 0.44 \\
%     & & body & 79.49 $\pm$ 0.56 & 92.94 $\pm$ 0.43 & 86.29 $\pm$ 0.56 & 55.78 $\pm$ 0.59 & 28.48 $\pm$ 0.43 \\
%     \hline
%     \multirow{8}{*}{50} & \multirow{2}{*}{Block1} & full & 61.33 $\pm$ 0.66 & 83.22 $\pm$ 0.58 & 73.01 $\pm$ 0.67 & 44.49 $\pm$ 0.49 & 25.34 $\pm$ 0.37 \\
%     & & body & 62.28 $\pm$ 0.67 & 83.91 $\pm$ 0.55 & 76.71 $\pm$ 0.57 & 49.21 $\pm$ 0.51 & 25.45 $\pm$ 0.40 \\ \cline{2-8}
%     & \multirow{2}{*}{Block2} & full & 69.85 $\pm$ 0.59 & 89.34 $\pm$ 0.46 & 81.05 $\pm$ 0.61 & 48.17 $\pm$ 0.50 & 27.17 $\pm$ 0.41 \\
%     & & body & 71.29 $\pm$ 0.63 & 90.54 $\pm$ 0.44 & 87.03 $\pm$ 0.51 & 53.84 $\pm$ 0.56 & 28.21 $\pm$ 0.42 \\ \cline{2-8}
%     & \multirow{2}{*}{Block3} & full & 79.28 $\pm$ 0.52 & 95.27 $\pm$ 0.31 & 87.75 $\pm$ 0.49 & 52.36 $\pm$ 0.47 & 32.10 $\pm$ 0.46 \\
%     & & body & 79.96 $\pm$ 0.55 & 95.00 $\pm$ 0.33 & 90.50 $\pm$ 0.43 & 59.09 $\pm$ 0.53 & 32.22 $\pm$ 0.43 \\ \cline{2-8}
%     & \multirow{2}{*}{Block4} & full & 86.34 $\pm$ 0.42 & 94.86 $\pm$ 0.34 & 81.80 $\pm$ 0.53 & 52.37 $\pm$ 0.56 & 32.32 $\pm$ 0.43 \\
%     & & body & 85.72 $\pm$ 0.45 & 96.78 $\pm$ 0.23 & 91.42 $\pm$ 0.39 & 62.86 $\pm$ 0.63 & 31.03 $\pm$ 0.44 \\
%     \hline
% \end{tabular}
% }\label{tab:subnetworks}
% \end{table}

\begin{table}[h]
\caption{Stage-wise 5-way $k$-shot accuracy (\%) of the features from a miniImageNet pre-trained model. An average pooling layer and an auxiliary classifier are attached at the end of each stage of ResNet10.}\label{tab:subnetworks}
\vspace{0.3cm}
\centering{%
\begin{tabular}{c|c|c|cccc|c}
    \toprule
    \multirow{2}{*}{Shot} & \multirow{2}{*}{Aux.} & Same-domain & \multicolumn{5}{c}{Cross-domain (BSCD-FSL)} \\
    \cmidrule{3-8}
     & & miniImageNet & CropDisease & EuroSAT & ISIC & ChestX & Mean \\
    \midrule
    \multirow{4}{*}{1} & Stage1 & 33.79{\stdfont $\pm$.68} & 46.66{\stdfont $\pm$.98} & 46.42{\stdfont $\pm$.82} & 26.77{\stdfont $\pm$.51} & 20.59{\stdfont $\pm$.28} & 35.11 \\
    & Stage2 & 39.31{\stdfont $\pm$.72} & 57.82{\stdfont $\pm$.94} & 54.05{\stdfont $\pm$.86} & 28.01{\stdfont $\pm$.52} & 20.84{\stdfont $\pm$.32} & 40.18 \\
    & Stage3 & 47.28{\stdfont $\pm$.80} & 65.69{\stdfont $\pm$.85} & 61.56{\stdfont $\pm$.90} & 30.07{\stdfont $\pm$.56} & 22.00{\stdfont $\pm$.38} & \textbf{44.83} \\
    & Stage4 & \textbf{51.88{\stdfont $\pm$.80}} & 65.73{\stdfont $\pm$.87} & 54.35{\stdfont $\pm$.92} & 30.42{\stdfont $\pm$.54} & 22.17{\stdfont $\pm$.37} & 43.17 \\
    \midrule
    \multirow{4}{*}{5} & Stage1 & 48.94{\stdfont $\pm$.75} & 72.82{\stdfont $\pm$.80} & 64.74{\stdfont $\pm$.74} & 34.92{\stdfont $\pm$.53} & 21.90{\stdfont $\pm$.35} & 48.60 \\
    & Stage2 & 56.40{\stdfont $\pm$.75} & 81.61{\stdfont $\pm$.62} & 73.65{\stdfont $\pm$.72} & 37.63{\stdfont $\pm$.51} & 22.65{\stdfont $\pm$.36} & 53.89 \\
    & Stage3 & 67.07{\stdfont $\pm$.70} & 88.19{\stdfont $\pm$.57} & 80.26{\stdfont $\pm$.64} & 40.87{\stdfont $\pm$.54} & 25.25{\stdfont $\pm$.41} & \textbf{58.64} \\
    & Stage4 & \textbf{74.61{\stdfont $\pm$.65}} & 88.68{\stdfont $\pm$.53} & 75.96{\stdfont $\pm$.67} & 42.97{\stdfont $\pm$.56} & 25.80{\stdfont $\pm$.43} & 58.35 \\
    \bottomrule
\end{tabular}
}
\end{table}

==> tex/02_introduction.tex <==
\section{Introduction}\label{sec:intro}

% 비교 그림
\begin{figure}[ht]
     \centering
     \begin{subfigure}[ht]{0.48\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/sec1/transfer_abs.pdf}
         \caption{Transfer \cite{bscd_fsl}}
         \label{fig:overview_transfer}
     \end{subfigure}
     \hfill
     \begin{subfigure}[ht]{0.48\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/sec1/simclr_abs.pdf}
         \caption{SimCLR}
         \label{fig:overview_simclr}
     \end{subfigure}
     
     \begin{subfigure}[ht]{0.48\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/sec1/transfer_simclr_abs.pdf}
         \caption{Transfer+SimCLR}
         \label{fig:overview_transfer_simclr}
     \end{subfigure}
     \hfill
     \begin{subfigure}[ht]{0.48\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/sec1/transfer_rr_simclr_abs.pdf}
         \caption{Transfer+RR+SimCLR (Ours)}
         \label{fig:overview_transfer_RR_simclr}
     \end{subfigure}
     \caption{Pre-training comparison between ours and three baselines. Classifiers are omitted.}
     \label{fig:overview_comparison}
\end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.7\linewidth]{figures/sec1/motivation.pdf}
%     \caption{Stage-wise 5way-$k$shot accuracy (\%) of the features from a miniImageNet pre-trained model. An average pooling layer and an auxiliary classifier are attached at the end of each stage of ResNet10.}
%     \label{fig:motivation}
% \end{figure}


% FSL 소개
Few-shot learning (FSL) has become an attractive field of research to tackle a small amount of labeled data problem with the development of deep learning. FSL aims to recognize novel classes in the target domain with a small number of samples using a model trained on base classes in the source domain with a large number of samples, where base classes and novel classes are disjoint. FSL has mainly been studied using meta-learning based and fine-tuning based approaches; meta-learning based approaches train models in an episodic manner (\ie, the few-shot evaluation procedure) \cite{maml, raghu2019rapid, oh2021boil, koch2015siamese, matchingnet, snell2017prototypical}, while fine-tuning based approaches train models in a mini-batch manner (\ie, the general supervised training procedure) \cite{chen2018a, Dhillon2020A, tian2020rethinking}. Such traditional FSL has generally addressed the situations where the source and target domains are similar.

% CD-FSL 소개 
\textbf{Problem: Source domain data that are similar to the target domain may not be sufficiently available in the real-world.} Cross-domain few-shot learning (CD-FSL) targets this concern. For instance, when few annotated satellite images exist, it is difficult to collect a large number of annotated images similar to them. In these situations, one has no choice but to use general source domain (\eg, ImageNet), which are very different from target domain (\eg, satellite images), to train models that can adapt to novel classes using few samples. Based on these situations, Guo \etal \cite{bscd_fsl} provided benchmark dataset for CD-FSL, named Broader Study of Cross-Domain Few-Shot Learning (BSCD-FSL). BSCD-FSL consists of four target domains where each domain has different characteristics according to perspective distortion, semantic contents, and color depth. It is also demonstrated that simple fine-tuning based approaches outperform all meta-learning based approaches on the BSCD-FSL benchmark \cite{bscd_fsl}.

% CD-FSL baselines (Transfer, SimCLR, Transfer+SimCLR)
\textbf{Three baselines for CD-FSL.} For CD-FSL, there are three representative baseline models depending on the pre-training dataset; Transfer (\ie, simple fine-tuning), SimCLR, and Transfer+SimCLR. \textbf{Transfer}, described in \Cref{fig:overview_transfer}, uses \emph{the labeled source dataset} to pre-train a network. This baseline does not use the target dataset. Recently, partial data in the target domain are usually used as unlabeled data before few-shot fine-tuning, which is a natural way because the model trained on the source domain does not guarantee performance on the target domain due to the gap of data distributions \cite{nsae}. \textbf{SimCLR}, described in \Cref{fig:overview_simclr}, uses \emph{the unlabeled target dataset} to pre-train a network based on NT-Xent loss (the normalized temperature-scaled cross-entropy loss) \cite{chen2020simple}, maximizing agreement between the two different augmented samples derived from the same sample. \textbf{Transfer+SimCLR}, described in \Cref{fig:overview_transfer_simclr}, uses \emph{both the labeled source dataset and unlabeled target dataset}. A network is first pre-trained on the labeled source dataset and then pre-trained once more on the unlabeled target dataset based on SimCLR. The difference between \textbf{SimCLR} and \textbf{Transfer+SimCLR} is that the former starts unsupervised pre-training from randomly initialized parameters, whereas the latter starts from the converged parameters on the source dataset. Islam \etal \cite{islam2021broad} demonstrated that \textbf{Transfer+SimCLR} generally showed the best performance because self-supervised learning makes more transferable representations than vanilla supervised learning and the combination with cross-entropy improves transfer learning performance.

% because \textbf{Transfer} focuses on the source dataset and \textbf{SimCLR} has a limitation on the number of unlabeled \emph{target domain} samples unlike unlabeled general samples.

% From DD paper,
% Table 1 shows the performance comparison of our approach with other methods on the BSCD-FSL benchmark. All models are trained on the miniImageNet dataset. “Transfer” denotes the baseline trained by cross-entropy loss on the base dataset. “SimCLR” is trained only on the unlabeled images. As noted by [10], self-supervised contrastive learning learns better transferable representation for a different downstream domain. Hence, we also create a “SimCLR(Base)” baseline that trains the encoder by optimizing self-supervised contrastive loss on the base dataset. “Transfer+SimCLR” refers to the model which is trained with supervised cross-entropy loss from the base dataset and self-supervised contrastive loss from the unlabeled target dataset, which has been reported to show superior transferability across domain [10]. STARTUP [22] is trained with three losses: cross-entropy loss on the base dataset, KL-divergence loss on the unlabeled dataset similar, and self-supervised contrastive loss on unlabeled images. STARTUP, Transfer+SimCLR and our approach use both the base dataset and additional unlabeled dataset during the representation learning phase.

% [10] A Broad Study on the Transferability of Visual Representations with Contrastive Learning


% pre-experiments
\textbf{Question: Is transfer of the pre-trained parameters on the source domain always good for the further training with target domain?}
To motivate our study, we investigate the stage-wise transferability of the network trained on the source dataset (\ie, miniImageNet) for FSL.\footnote{The details of experimental setup are explained in \Cref{subsec:setup}.} \Cref{tab:subnetworks} summarizes the few-shot task accuracy evaluated on the target dataset, using the intermediate output features after each stage of ResNet10. Stage-wise intermediate features are classified by a fine-tuned auxiliary classifier, as proposed in \cite{teerapittayanon2016branchynet,zhang2019your,zhang2019scan}. For instance, `Stage1' in `Aux.' means that the output of Stage1 is fed into average pooling and then classified by an auxiliary classifier. The results present that in-depth representations are consistently better with a large margin under the same domain, however, this trend collapses in the last stage when the target domain differs from the source domain (\ie, cross-domain). It implies that \emph{transferring (or, reusing) the last stage of models trained on the source domain may be inappropriate for the target domain if domain differences appear.}

\input{tables/subnetworks}

% 제안하는 방법 + 이전 approaches와의 차이점
\textbf{Novel baseline for CD-FSL with unlabeled target data.}
Inspired by the above observations, we propose a simple yet powerful method; we re-randomize the top layers of an extractor after pre-training on the source dataset, then train the re-randomized models using the unlabeled target data based on SimCLR. We express it \textbf{Transfer+RR(Re-Randomization)+SimCLR}, described in \Cref{fig:overview_transfer_RR_simclr}. Our proposed method outperforms recent CD-FSL algorithms such as STARTUP \cite{phoo2021selftraining} and Dynamic Distillation \cite{islam2021dynamic}. Prior studies focused on how to leverage the unlabeled target dataset efficiently, combining knowledge distillation \cite{hinton2015distilling}. However, we further consider \emph{the removal of fitted parameters on the source domain}. We believe that our re-randomized baseline model will lay the groundwork of linking between transfer in CD-FSL and recent works of self-supervised learning.
%Moreover, it is intuitively explained that our proposed method is in-between \textbf{SimCLR} and \textbf{Transfer+SimCLR} from the SimCLR learning's initialization perspective.
% Ours maintain rich general information from source dataset as Transfer+SimCLR, while starting from random initialization as SimCLR to obtain target-specific parameters. 
Our contributions are summarized as follows:
\begin{itemize}[leftmargin=*]
    \item We propose a simple yet powerful method, \textbf{Transfer+RR+SimCLR}, which re-randomizes a high-level extractor before SimCLR pre-training. The intuition behind this method is explained by removing the fitted parameters on the source dataset.
    \item We show that the re-randomization reduces the workload of SimCLR pre-training and that re-randomized initialization at top layers makes loss landscape smoother than entirely random (SimCLR) or converged (Transfer) initialization.
    \item We investigate the effect of augmentation policies during SimCLR pre-training on the performance.
    \item We demonstrate the effectiveness of re-randomization itself for CD-FSL when unlabeled target data is not available and analyze where and how to re-randomize in detail.
\end{itemize}

% Assuming accessibility to samples in the target domain, two-stage teacher-student pre-training is used to extract sophisticated representations from unlabeled target data \cite{phoo2021selftraining, islam2021dynamic}.

% STARTUP 발췌 내용
% Baselines. We compare to the techniques reported in Guo et al. (2020), which includes most state of-the-art approaches as well as a cross-domain few-shot technique Tseng et al. (2020). The top performing among these is naive Transfer which simply trains a convolutional network to classify the base dataset, and uses the resulting representation to learn a linear classifier when faced with novel few-shot tasks. These techniques do not use the novel domain unlabeled data. We also compare to another baseline, SimCLR that uses the novel domain unlabeled data to train a representation using SimCLR(Chen et al., 2020), and then uses the resulting representation to learn linear classifiers for few-shot tasks. This builds upon state-of-the-art self-supervised techniques. To compare to a baseline that uses both sources of data, we establish Transfer + SimCLR. This baseline is similar to the SimCLR baseline except the embedding is initialized to Transfer’s embedding before SimCLR pre-training.

%\textcolor{red}{Intuitively, rather than incorporating additional unlabeled data from the target domain to aid in fine-tuning, we turn our attention to unwanted source data in pre-trained models.}
% \textcolor{blue} {
% Intuitively, rather than incorporating additional unlabeled data from the target domain to aid in fine-tuning, we consider the removal of unwanted source data in pre-trained models.
% First, we consider the batch normalization (BN) statistics. It has been shown in the domain adaptation context that one needs to modulate the statistical information of the source domain before applying the model to the target domain. Therefore, we consider various methods to reset the BN statistics learned from the source domain, without hurting model stability.
% Secondly, we selectively adopt the pre-trained weights, in a layer-wise manner. In general, the extractor, \ie, body, contains general image feature information while the classifier, \ie head, contains class-specific information. However, under extreme domain differences, it is believed that the features learned in the upper-layers of the pre-trained extractor may be unsuited for the target domain. Based on this intuition, we selectively adopt weights from the lower layers of the pre-trained classifier and re-randomize the remaining layers for fine-tuning on the target domain.
% }
% model stability part is related to initialization-related hypothesis by Namgyu
%우리의 방식은 pre-training 시 target domain 을 사용하는 것 (like prior works) 이 아닌, fine-tuning 시 source domain에 대한 정보를 일부분 버리는 전략을 바탕에 둡니다.
% We first revisit batch normalization (BN) in domain adaptation context, where one needs to modulate the statistical information of source domain before moving to target domain. From the observations, we \textbf{replace the BN layers' running statistics from the source domain with target domain statistics}.
% what observations?
% Furthermore, in general, an extractor (\ie, body) represents general features at the low-level, while represents specific features at the high-level. /textcolor{blue}{Under extreme differences between the source and target  domains, it is believed that the upper-layers of the pre-trained extractor may be unsuitable for use in the target domain.}
% Based on this intuition, \textbf{this portion is re-randomized before fine-tuning along with classifier initialization} (re-randomization in \Cref{fig:overview}).
% Finally, we show that \textbf{XXXX} provides comparable or better performance even without using unlabeled target data and that \textbf{XXXX} can be applied to the prior methods using unlabeled target data (such as \cite{phoo2021selftraining, islam2021dynamic}), outperforming the state-of-the-art performance.






==> tex/05_methods.tex <==
\section{Main approach: RESET}\label{sec:methods}

In this section, we explain \algname{} in three steps following the learning pipeline; pre-training on labeled source data $D_B$ (\cref{sec:methods_1}), re-randomizing the upper layers of the backbone extractor (\cref{sec:methods_2}), and self-supervised training on unlabeled target data $D_N^U$ (\cref{sec:methods_3}). The final pre-trained network is fine-tuned on the support set $D_s$ and evaluated on the query set $D_q$. Note that SimCLR \cite{chen2020simple}, one of the baselines for self-supervised learning, is used for step 3 due to its simplicity and expandablity.

% A model is first pre-trained on the labeled source data $D_B$ (\cref{sec:methods_1}). Prior to further training, the backbone extractor is partially re-randomized at top layers (\cref{sec:methods_2}). Subsequently, the re-randomized network is pre-trained once more on the unlabeled target data $D_N^U$ in a self-supervised manner, in which we use SimCLR \cite{chen2020simple} for our study due to simplicity (\cref{sec:methods_3}). Finally, the pre-trained network is fine-tuned using the support set $D_s$ (\ie,  few-shot labeled target data) and evaluated on query set $D_q$. (\cref{sec:methods_1}) 
%Our contribution is in the introduction of the second step, \ie, re-randomization, as a simple yet effective method on top of the existing pipeline. We explain the details of each step in the following subsections.

% 각 subsection 마다 방법 설명 + 주목하는 부분에 대한 설명 2 단락으로 구성
\subsection{Pre-training on $D_B$}\label{sec:methods_1} 
% FSL downstream task using $D_N^L$
A model $C_1 \circ f$ is pre-trained on labeled source data $D_B$ by minimizing cross-entropy loss in a mini-batch manner, where $f$ is a backbone that maps input $x$ into representation $z \in \mathbb{R}^{d}$ and $C_1 \in \mathbb{R}^{K \times d}$ is a linear classifier. In general, a large dataset is used as $D_B$, the number of classes $K$ is large (\eg, if ImageNet is $D_B$, then $K$ is 1000). At the end of this stage, the classifier $C_1$ is removed.

% 아래 문단 수정
However, a simple fine-tuning method has a limitation for CD-FSL because the pre-trained $f$ may fail to extract meaningful representations for the different target domains. In CD-FSL, the main objective of pre-training is transferability of representations. Islam \etal \cite{islam2021broad} demonstrated that representations learned via cross-entropy loss contain high-level semantics that are not transferable to different domains. This characteristic prevents the pre-trained model from rapidly adapting to a novel task. Simultaneously, this motivates the next step, re-randomization for removing source-fitted semantics.

% Here, we focus on transferability of representations, which is the objective of pre-training. Islam \etal \cite{islam2021broad} demonstrated that representations learned via cross-entropy loss contain more high-level semantics than those learned via contrastive loss. This characteristic prevents pre-trained models from rapid adaptation to a novel task. It implies that a simple fine-tuning method has a limitation for CD-FSL because the pre-trained $f$ through this step may fail to extract meaningful representations for the different target domains. Furthermore, this motivates the next step, re-randomization for removing source-fitted semantics.

% The objective of pre-training is to develop a backbone network that extracts meaningful representations. In this stage, a linear classifier for many classes (\eg, 1000 classes for ImageNet) is required after a backbone network. An initialized model $f_{\theta_0}$ is pre-trained using large labeled source dataset $D_B$ (\eg, miniImageNet, tieredImageNet, and ImageNet) by minimizing the cross entropy loss in a mini-batch manner. After pre-training, the classifier is removed.

% FSL downstream task is divided into two steps: (1) fine-tuning using $D_s$ and (2) evaluation using $D_q$.
% For fine-tuning, we construct an episodic batch with the labeled target dataset by sampling $(D_s, D_q)$ from $D_N^L$, as in the FSL statement of \Cref{sec:problem_statement}. In this stage, a new linear classifier for few classes (\eg, 5 classes) is attached after the pre-trained backbone. The backbone attached with a new classifier is trained using the support set $D_s$ (\ie, few labeled target dataset) in a mini-batch manner.
% When the fine-tuning is over, the model is evaluated on $D_q$ with these running statistics. Note that each episode is an independent process, thus the fine-tuned model is reset for every new episode. 
% This pre-training and fine-tuning procedure is analogous to transfer learning, thus called \textbf{Transfer} (\Cref{fig:overview_transfer}) from \cite{bscd_fsl}.

\subsection{Re-randomization of the backbone $f$}\label{sec:methods_2}
We re-randomize the upper layers of the pre-trained backbone $f$ through step 1 to reset source-fitted parameters. Specifically, the weights\footnote{The biases of convolutional layers are not used.} of convolutional layers are re-randomized by the values sampled from uniform distribution\footnote{This randomization method is the default setting in PyTorch \cite{paszke2019pytorch}.} \cite{he2015delving}. The scaling and shifting parameters of batch normalization layers are re-randomized by ones and zeros, respectively.

The reason why ``upper'' layers of backbone $f$ are re-randomized is that more domain-specific representations are extracted as the depth increases in convolutional neural networks \cite{yosinski2014transferable, reinit_cnn, raghu2019transfusion, maennel2020neural}. Re-randomization or re-initialization of upper layers helps training loss to escape from local minima based on $D_B$ and allows bottom-level layers to be sufficiently updated, alleviating the gradient vanishing problem \cite{ro2019backbone, li2020rifle}. Such effectiveness of re-randomization matches the favorable characteristic in CD-FSL, representation change \cite{feature_transformation, oh2021boil}.

% In \textbf{Transfer+SimCLR}, pre-training with large source dataset plays a role as an initialization of self-supervised learning. However, many prior works have demonstrated that these pre-trained backbones based on $D_B$ fail to extract meaningful representations on the target domain, in particular under the extreme domain differences. This is because the pre-trained backbones are fitted on the source domain at the high-level extractor, not on the target domain. In general, the deeper the depth, the more specific representation for classification is extracted \cite{yosinski2014transferable, reinit_cnn, raghu2019transfusion, maennel2020neural}. 

% Inspired by the above observations, we suggest that the upper layers of the pre-trained backbone should be re-randomized to reset the parameters fitted on the source domain. This intuition matches with prior works \cite{feature_transformation, oh2021boil} that highlighted representation change, in particular under CD-FSL. By re-randomizing the upper layers, the pre-trained backbone can escape local minima based on $D_B$ and be updated with amplified gradients for the target domain \cite{li2020rifle}, leading to representation change. We insert the re-randomization step between pre-training with $D_B$ and SimCLR pre-training with $D_N^U$, and call this re-randomized baseline \textbf{Transfer+RR(Re-Randomization)+SimCLR} (\Cref{fig:overview_transfer_RR_simclr}). 

% Specifically, we re-randomize the convolutional layers (Conv) via sampling from uniform distribution \cite{he2015delving} and the Batch Normalization layers (BN) as ones of scaling parameters and zeros of shifting parameters.

% In summary, \textbf{Transfer+RR+SimCLR} is in-between \textbf{SimCLR} (\Cref{fig:overview_simclr}) and \textbf{Transfer+SimCLR}; it starts SimCLR pre-training from the mixture of a random backbone at the upper layers as \textbf{SimCLR} and the pre-trained backbone at the bottom layers as \textbf{Transfer+SimCLR}.

\subsection{Self-supervised training on $D_N^U$}\label{sec:methods_3}
% target domain data 만 쓴다는 것..
The re-randomized backbone $f$ is trained fully based on one of the self-supervised methods such as MoCo\cite{he2020momentum}, BYOL\cite{grill2020bootstrap}, and SimCLR\cite{chen2020simple}.\footnote{We call this step SimCLR pre-training to distinguish from step 1 pre-training.} The reason why self-training the re-randomized backbone entirely is that re-randomization amplify gradients such that low-level can be updated. For our study, SimCLR is used due to simplicity. Namely, a model $C_2 \circ f$ is pre-trained on \emph{unlabeled target data} $D_N^U$ by minimizing NT-Xent loss, where $C_2$ is a two-layer projection MLP, consisting of linear, ReLU, and linear layers. The former linear layer is in $\mathbb{R}^{d \times d}$ and the latter one is in $\mathbb{R}^{p \times d}$, where $p$ is the dimension of projection. At the end of this stage, the projection MLP $C_2$ is removed.

\algname{} reduces to SimCLR if step 1 and 2 are omitted and to TranSimCLR if step 2 is omitted. From the SimCLR's initialization perspective, \algname{} can be thought an algorithm in-between SimCLR and TranSimCLR. Namely, \algname{} starts SimCLR pre-training from the mixture of a random backbone at the upper layers as SimCLR and the pre-trained backbone at the bottom layers as TranSimCLR.

To evaluate the final pre-trained backbone $f$ through step 1 to 3, a classifier $g \in \mathbb{R}^{n \times d}$ is fine-tuned on support set $D_s$ based on representations extracted by $f$, where $n$ is the number of classes for few-shot tasks (in general, 5). Finally, the fine-tuned model $g \circ f$ is evaluated on query set $D_q$.

% FSL downstream task is divided into two steps: (1) fine-tuning using $D_s$ and (2) evaluation using $D_q$.
% For fine-tuning, we construct an episodic batch with the labeled target dataset by sampling $(D_s, D_q)$ from $D_N^L$, as in the FSL statement of \Cref{sec:problem_statement}. In this stage, a new linear classifier for few classes (\eg, 5 classes) is attached after the pre-trained backbone. The backbone attached with a new classifier is trained using the support set $D_s$ (\ie, few labeled target dataset) in a mini-batch manner.
% When the fine-tuning is over, the model is evaluated on $D_q$ with these running statistics. Note that each episode is an independent process, thus the fine-tuned model is reset for every new episode. 
% This pre-training and fine-tuning procedure is analogous to transfer learning, thus called \textbf{Transfer} (\Cref{fig:overview_transfer}) from \cite{bscd_fsl}.


% pre-trained more based on SimCLR \cite{chen2020simple}. To distinguish this step from the prior pre-training step, we call it SimCLR pre-training. In general, SimCLR requires significantly many samples to obtain elaborate representations. However, this condition is not satisfied in our problem setting, and hence pre-training using $D_B$ precedes. Placing this step between the pre-training and fine-tuning in \Cref{sec:methods_1} is called \textbf{Transfer+SimCLR} (\cref{fig:overview_transfer_simclr}), which was suggested as one of the baselines in \cite{phoo2021selftraining}.

% In summary, \textbf{Transfer+RR+SimCLR} is in-between \textbf{SimCLR} (\Cref{fig:overview_simclr}) and \textbf{Transfer+SimCLR}; it starts SimCLR pre-training from the mixture of a random backbone at the upper layers as \textbf{SimCLR} and the pre-trained backbone at the bottom layers as \textbf{Transfer+SimCLR}.






\iffalse
\subsection{Pre-training using $D_B$}\label{sec:methods_1}
The objective of pre-training is to develop a backbone network that extracts meaningful representations. In this stage, a linear classifier for many classes (\eg, 1000 classes for ImageNet) is required after a backbone network. An initialized model $f_{\theta_0}$ is pre-trained using large labeled source dataset $D_B$ (\eg, miniImageNet, tieredImageNet, and ImageNet) by minimizing the cross entropy loss in a mini-batch manner. However, many prior works have demonstrated that these pre-trained backbones fail to extract meaningful representations on the target domain, in particular under the extreme domain differences. This is because the pre-trained backbones based on $D_B$ are fitted on the source domain at the high-level extractor, not on the target domain. In general, the deeper the depth, the more specific representation for classification is extracted \cite{yosinski2014transferable, reinit_cnn, raghu2019transfusion, maennel2020neural}. After pre-training, the classifier is removed.

\subsection{Re-randomization: partially removing source-specific information}\label{sec:methods_2}
Inspired by the above observations, we suggest that the high-level extractor of the pre-trained backbone should be also re-randomized to remove the parameters fitted on the source domain. This intuition matches with prior works \cite{feature_transformation, oh2021boil} that highlighted representation change, in particular under CD-FSL. By re-randomizing the high-level extractor, the pre-trained backbone can escape local minima based on $D_B$ and be updated with amplified gradients for the target domain \cite{li2020rifle}, leading to representation change.

Specifically, we re-randomized the convolutional layers (Conv) via sampling from uniform distribution (cite, He) and the Batch Normalization layers (BN) with scaling parameters as ones and shifting parameters as zeros.


\subsection{Pre-training using $D_N^U$ based on SimCLR}\label{sec:methods_3}
Re-randomized models are pre-trained more based on SimCLR \cite{chen2020simple}. To distinguish this step from the first pre-training step, we call it SimCLR pre-training. SimCLR is the method that maximizes agreement between the two different augmented samples from the same unlabeled sample. In general, SimCLR requires significantly many samples to elaborate representations. However, this condition is not satisfied in our problem setting, and hence pre-training using $D_B$ precedes.

In this stage, there is difference on initialization points among \textbf{SimCLR}, \textbf{Transfer+SimCLR}, and \textbf{Transfer+RR+SimCLR} (Ours). \textbf{SimCLR} starts from a random backbone, whereas \textbf{Transfer+SimCLR} starts from the pre-trained backbone using $D_B$. Our method, \textbf{Transfer+RR+SimCLR} starts from the mixture of the pre-trained backbone at the low- and mid-level and a random backbone at the high-level backbone. 

\subsection{Fine-tuning using $D_s$ and Evaluation using $D_q$}\label{sec:methods_4}
For fine-tuning, we construct an episodic batch with the labeled target dataset by sampling $(D_s, D_q)$ from $D_N^L$, as in the FSL statement of \Cref{sec:problem_statement}. In this stage, a new linear classifier for few classes (\eg, 5 classes) is attached after the pre-trained backbone. The backbone attached with a new classifier is trained using the support set $D_s$ (\ie, few labeled target dataset) in a mini-batch manner.
%When the fine-tuning is over, we propose an additional trick; update running statistics in batch normalization layers using unlabeled target dataset. Because running statistics (\ie, accumulated mean and variance in a moving average way) in batch normalization layers are accumulated by few samples during fine-tuning, they can be unstable for generality. We can replace them with running statistics through unlabeled target dataset (at least more than $nk$ samples), regardless of sampled few-shot images.  Finally, the fine-tuned model is evaluated on $D_q$ with these running statistics. 
When the fine-tuning is over, the model is evaluated on $D_q$ with these running statistics. Note that each episode is an independent process, thus the fine-tuned model is reset for every new episode.
\fi

% \input{tables/clustering}


%  \subsection{Motivation}\label{subsec:PRE}


% We further investigate the relative change of parameters per layer and show that the performance improvement through fine-tuning attributes to a classifier even though the entire network is fine-tuned. In \cite{bscd_fsl}, although it is shown that the more transferable layers in the extractor exist using the relative change, a classifier layer is not addressed. We follow the proposed method in \cite{bscd_fsl} to calculate the relative change, \ie, $\frac{\norm{\theta-\theta_f}}{\norm{\theta}}$, where $\theta$ and $\theta_f$ are parameters before and after fine-tuning, respectively. \Cref{fig:baseline_relative_change} describes the relative change of parameters per layer including a classifier. It is observed that the change in the extractor is significantly less than that in the classifier.

% Furthermore, this characteristic is also demonstrated in terms of performance. \Cref{tab:intro_result} describes 5-way 5-shot test accuracy before and after fine-tuning in both parametric and non-parametric ways. A parametric way indicates the evaluation using a learnable reinitialized and fine-tuned classifier, while a non-parametric way indicates the evaluation using the nearest classifier based on extracted representations. It is shown that, with a non-parametric classifier, there is little change between before and after fine-tuning except for CropDisease. In addition, the performance gap between with a parametric and non-parametric classifier implies that fine-tuning attributes to a classifier even though the entire network is fine-tuned.

% \begin{table}[ht]
% \caption{5-way 5-shot test accuracy over 600 tasks on miniImageNet $\rightarrow$ \{miniImageNet, BSCD-FSL\}. ResNet10 is used and mean and 95\% confidence interval are reported. A non-parametric classifier means the nearest classifier.}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{c|cc|cc}
%     \hline
%     evaluation & \multicolumn{2}{c|}{with a non-parametric classifier} & \multicolumn{2}{c}{with a parametric classifier} \\
%     \hline
%     fine-tuning & before & after & before & after \\
%     \hline
%     miniImageNet & 47.41 $\pm$ 1.08 & 47.17 $\pm$ 1.05 & 19.78 $\pm$ 0.47 & 74.04 $\pm$ 0.65 \\
%     CropDisease  & 48.13 $\pm$ 1.09 & 64.19 $\pm$ 1.22 & 19.96 $\pm$ 0.57 & 88.62 $\pm$ 0.52 \\
%     EuroSAT      & 55.10 $\pm$ 0.86 & 54.31 $\pm$ 0.91 & 20.30 $\pm$ 0.60 & 79.10 $\pm$ 0.61 \\
%     ISIC         & 33.31 $\pm$ 0.52 & 33.89 $\pm$ 0.63 & 20.03 $\pm$ 0.39 & 49.10 $\pm$ 0.59 \\
%     ChestX       & 22.72 $\pm$ 0.31 & 23.16 $\pm$ 0.33 & 19.87 $\pm$ 0.28 & 26.10 $\pm$ 0.41 \\
%     \hline
% \end{tabular}
% }\label{tab:intro_result}
% \end{table}

% \begin{table}[ht]
% \caption{5-way 5-shot test accuracy over 600 tasks on miniImageNet $\rightarrow$ \{miniImageNet, BSCD-FSL\} of pre-trained model according to the reinitialization ratio $r$ of zero reinitialization in the last block in a non-parameteric manner. ResNet10 is used and mean and 95\% confidence interval are reported.}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{c|ccccc}
%     \hline
%     $r$ & miniImageNet & CropDisease & EuroSAT & ISIC & ChestX \\
%     \hline
%     0.0 & 47.41 $\pm$ 1.08 & 48.13 $\pm$ 1.09 & 55.10 $\pm$ 0.86 & 33.31 $\pm$ 0.52 & 22.72 $\pm$ 0.31 \\
%     0.2 & 47.10 $\pm$ 0.91 & 48.23 $\pm$ 1.15 & 57.14 $\pm$ 0.86 & 27.70 $\pm$ 0.45 & 22.38 $\pm$ 0.32 \\
%     0.5 & 47.53 $\pm$ 0.90 & 44.27 $\pm$ 1.16 & 50.33 $\pm$ 1.16 & 25.05 $\pm$ 0.39 & 21.97 $\pm$ 0.31 \\
%     0.8 & 36.83 $\pm$ 0.79 & 39.17 $\pm$ 1.07 & 46.37 $\pm$ 0.92 & 23.90 $\pm$ 0.37 & 20.38 $\pm$ 0.16 \\
%     1.0 & 20.00 $\pm$ 0.00 & 20.00 $\pm$ 0.00 & 20.00 $\pm$ 0.00 & 20.00 $\pm$ 0.00 & 20.00 $\pm$ 0.00 \\
%     \hline
% \end{tabular}
% }\label{tab:zero_reinit}
% \end{table}

% Fine-tuning으로 인한 extractor improve보다 classifier의 improve만 두드러짐.

% We suggest re-randomization $RR(p, m)$, where $p$ indicates the position of re-randomization and $m$ indicates the re-randomization method. Re-randomized parameters on the extractor must be learned during fine-tuning to achieve the desired performance.

% For convolution layers,

% For batcch normalization layers,


% For convolution layers, the weight shape is $(d_{out}, d_{in}, K, K)$ in general, where $K$ is the kernel size and $d_{in}$ and $d_{out}$ are the number of channels of input and output feature map, respectively. Convolution layers can be reinitialized in a element-wise or channel-wise manner. Note that we focus on channel-wise reinitialization approaches because each channel involves each characteristic and channel-wise reinitialization approaches outperform element-wise reinitialization approaches (\Cref{subsubsec:how_to_reinit}). In the case of channel-wise method, $r$ can be decoupled into $r_{in}$ and $r_{out}$, where $r_{in}$ and $r_{out}$ are the reinitialization ratio on $d_{in}$ and $d_{out}$, respectively. If $r_{in}$ \emph{or} $r_{out}$ is 1.0 on a convolution layer, parameters of this layer is completely reinitialized. On the other hand, if $r_{in}$ \emph{and} $r_{out}$ are 0.0 on a convolution layer, parameters of this layer is completely reused. Otherwise, only $(1-r_{in})(1-r_{out})$ times all pre-trained parameters are reused.

% For the next batch normalization layer following a convolution layer, scaling and shifting parameters are reinitialized as 1.0 and 0.0, respectively, on entirely reinitialized channels, \ie, $r_{out}D_{out}$. \Cref{fig:reinit_fig} describes channel-wise reinitialization on a convolution layer and a batch normalization layer. The green cubic represents pre-trained parts using labeled source domain dataset, while the white cubic represents reinitialized parts. 

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figures/sec4/reinit_detail.pdf}
%     \caption{Channel-wise reinitialization on a convolution layer and a batch normalization layer.}
%     \label{fig:reinit_fig}
% \end{figure}

% 일반화된 방법으로 식, 표현을 적어 놓고 experiment에서 high-level의 init이 중요함을 보여야 함
% 이 방법을 떠오르게 된 계기까지의 흐름이 있어야 할 듯


% Note that when the domain gap is large, the low- and middle-level extractors are frozen and high-level extractors are fine-tuned in general fine-tuning methods, however, the initialization point of these methods is the pre-trained model, whereas that of our methods is a random re-initialized model.

